Identifiability Guarantees for Causal Disentanglement from Soft Interventions

Causal disentanglement aims to uncover a representation of data using latent variables that are interrelated through a causal model. Such a representation is identifiable if the latent model that explains the data is unique. In this paper, we focus on the scenario where unpaired observational and interventional data are available, with each intervention changing the mechanism of a latent variable. When the causal variables are fully observed, statistically consistent algorithms have been developed to identify the causal model under faithfulness assumptions. We here show that identifiability can still be achieved with unobserved causal variables, given a generalized notion of faithfulness. Our results guarantee that we can recover the latent causal model up to an equivalence class and predict the effect of unseen combinations of interventions, in the limit of infinite data. We implement our causal disentanglement framework by developing an autoencoding variational Bayes algorithm and apply it to the problem of predicting combinatorial perturbation effects in genomics.

==> content/old/append-a.tex <==
\subsection{Known Latent Dimension}

Consider an easier setting where the dimension $p$ of the latent causal variable $U$ is known and we have data from exactly one hard intervention per latent node. In other words, $K=p$ in Corollary \ref{cor:1}. We will generalize the discussion to unknown $p$ in the next section. For $K=p$, the identifiability result of hard interventions can be deduced from \cite{ahuja2022interventional}. For completeness, we present full proof here.

\begin{proof}[Proof of Corollary \ref{cor:1} ($K=p$)]
We show $\langle U,\cG,I_1,...,I_p\rangle$ is identifiable up to its $\cM$-equivalence class by two steps: (Step 1) following \cite{ahuja2022interventional}, we prove that $\langle U,I_1,...,I_p\rangle$ can be identified up to its $\cM$-equivalence class, (Step 2) we then show that $\cG$ is identifiable up to permutation that is consistent with the permutation of $U$.  

\textbf{Step 1:} $\langle U,I_1,...,I_p\rangle$ can be recovered up to its $\cM$-equivalence class by any mapping $\hat{g}:\bbR^n\rightarrow \bbR^{p}$ that satisfies two conditions: (1) there exists a full row rank polynomial\footnote{This is defined the same as in Assumption \ref{assumption:1}.2.} $\hat{f}(\cdot)$ such that $\hat{f}\circ\hat{g}(X)=X$ for all $X\in \cD\cup\cD^1\cup ...\cup\cD^p$; (2) for each $i\in [p]$, $\hat{g}(X)_i$, the $i$-th entry of $\hat{g}(X)$, is a constant for all $X\in\cD^i$. In other words, the variables $\hat{U}:=\hat{g}(X)$ given by $\hat{g}$ that satisfies (1) and (2) above must be such that $\hat{U}_{\pi(i)}=\lambda_i U_i+b_i$ for all $i\in [p]$, where $\pi$ is a permutation of $[p]$, coefficients $\lambda_1,...,\lambda_p$ are nonzero, and $b_1,...,b_p$ are constant intercepts. In addition, this identifies intervention targets $\hat{I}_i$ of $\cD^i$ such that $\hat{I}_i=\pi(I_i)$.
 
\begin{quote}
\textit{Proof of Step 1:}
First, there exists a solution to conditions (1) and (2) by $\hat{g}=M_{\tau}\circ f^{-1}$, where $f$ is ground-truth mapping (it is invertible based Assumption \ref{assumption:1}.2) and $M_{\tau}$ is a permutation operation such that $M_{\tau}(V)=(V_{\tau(1)},...,V_{\tau(p)})$ for all $V\in \bbR^p$. Here $\tau(i)$ is the latent node that is being intervened to obtain $\cD^i$. To see that $\hat{g}$ satisfies (1): set $\hat{f}=f\circ M_\tau^{-1}$, then $\hat{f}\circ \hat{g}(X)=f\circ M_\tau^{-1}\circ M_{\tau}\circ f^{-1} (X)=X$. To see that $\hat{g}$ satisfies (2): since $\cD^i$ corresponds to a hard intervention on $U_{\tau(i)}$, we have $\hat{g}(X)_i=(M_\tau\circ f^{-1}(X))_i=f^{-1}(X)_{\tau(i)}=U_{\tau(i)}$ which is a constant for $X\in\cD^i$.

Now suppose that $\hat{g}:\bbR^n\rightarrow\bbR^p$ satisfies conditions (1) and (2) where $\hat{f}$ is the corresponding mapping in (1). Write $\hat{f}(U)=(U,\kpd U^2,..., \kpd U^{\hat{d}})\hat{H}+\hat{h}$ for some integer $\hat{d}$, a full row rank matrix $\hat{H}\in\bbR^{(p+...+p^{\hat{d}})\times n}$, and a vector $\hat{h}\in\bbR^{n}$. For $X\in\cD\cup\cD^1\cup...\cup\cD^p$, denote $\hat{g}(X)$ as $\hat{U}$ and $f^{-1}(X)$ as $U$ respectively. From (1), we have
\begin{equation}\label{cor:eq-1}
    (\hat{U},\kpd \hat{U}^2, ..., \kpd \hat{U}^d)\hat{H} + \hat{h} =\hat{f}\circ\hat{g}(X)=X=f\circ f^{-1}(X)= (U,\kpd U^2,..., \kpd U^d)H+h.
\end{equation}
Since $\hat{H}$ has full row rank, it has pseudo-inverse $\hat{H}^{\dagger}\in\bbR^{n\times(p+p+...p^{\hat{d}})}$ such that $\hat{H}\hat{H}^{\dagger}$ is the identity matrix. Multiplying Eq.\eqref{cor:eq-1} by $\hat{H}^{\dagger}$ on both sides, we have
\[
(\hat{U},\kpd \hat{U}^2, ..., \kpd \hat{U}^{\hat{d}}) = (U,\kpd U^2,..., \kpd U^d)H\hat{H}^{\dagger}+(h-\hat{h})\hat{H}^{\dagger}.
\]
Taking the first $p$ columns, we know that $\hat{U}$ can be written as a polynomial of $U$ (denote as $\hat{U}=poly_1(U)$). Similarly, since $H$ has full row rank, we can multiply Eq.\eqref{cor:eq-1} by its pseudo-inverse $H^{\dagger}$ on both sides and arrive at the fact that $U$ can be written as a polynomial of $\hat{U}$ (denote as $U=poly_2(\hat{U})$). Therefore we have $U=poly_2(poly_1(U))$ for all $U\in\bbU$. Since $\bbU^{\circ}$ is non-empty, we know that $U=poly_2(poly_1(U))$ on some open set. By the fundamental theorem of algebra \cite{fine1997fundamental}, we know that $poly_1$ and $poly_2$ must have degree $1$. Thus $\hat{U}=U\Lambda + B$ for some non-singular matrix $\Lambda$ and vector $B$.

Finally, since $\hat{g}$ satisfies (2), for $i\in [p]$, we have $\hat{g}(X)_i=\hat{U}_i=U\Lambda_{:,i}+B_i$ as a constant for all $X\in\cD^i$. Suppose $\cD^i$ corresponds to the hard intervention on $U_{\tau(i)}$ and denote the support of $U$ from $\bbP_U^{\{\tau(i)\}}$ as $\bbU^{i}$. Since $\bbU^{i}$ has non-empty interior on all nodes aside from $U_{\tau(i)}$, we know that there exists $U\in \bbU^{i}$ and $\epsilon>0$ such that $U+\epsilon E_j\in \bbU^i$ for all $j \neq \tau(i)$, where $E_j$ is the one-hot vector with the $j$-th entry being one. Since $(U+\epsilon E_j)\Lambda_{:,i}+B_i$ is a constant that equals to $U\Lambda_{:,i}+B_i$ for all $j \neq \tau(i)$, it means $\Lambda_{j,i}=0$ for all $j \neq \tau(i)$. Thus,
\[\hat{U}_i=\Lambda_{\tau(i),i}U_{\tau(i)}+B_i,\]
for all $i\in [p]$. Since $\Lambda$ is non-singular, we have $\Lambda_{\tau(i),i}\neq 0$. Let $\pi$ be the permutation such that $M_{\pi}=M_{\tau}^{-1}$, $\lambda_{i}=\Lambda_{i,\pi(i)}\neq 0$, and $b_i=B_{\pi(i)}$. We proved that mapping $\hat{g}$ gives $\hat{U}=\hat{g}(X)$ such that $\hat{U}_{\pi(i)}=\lambda_i U_i+b_i$ for all $i\in [p]$. In addition, let $\hat{I}_i=\{i\}$; since $\cD^i$ corresponds to intervening on $U_{\tau(i)}$ and $M_{\pi}=M_{\tau}^{-1}$, we have $\hat{I}_i=\pi(\{\tau(i)\})=\pi(I_i)$. Step 1 is proven.
\end{quote}

\textbf{Step 2:} let $\hat{g}$ be the solution to step 1, then it gives variables $\hat{U}_{\pi(i)}=\lambda_i U_i+b_i$ with $\lambda_i\neq 0$ and all $i\in [p]$. Since $\lambda_i\neq 0$, $\bbP_{U}$ induces a distribution $\bbP_{\hat{U}}$ that is Markov with respect to $\cG_{\pi}$. Here $\cG_{\pi}$ is defined the same as the main text with $\pi(i)\rightarrow \pi(j)\in\cG_{\pi}$ if and only if $i\rightarrow j \in \cG$. We show that $\cG_{\pi}$ is identifiable. 

\begin{quote}
\textit{Proof of Step 2:}
From the proof above, we know that $\cD^i$ corresponds to setting $U_{\tau(i)}$, or equivalently $\hat{U}_i$, to a fixed value. Therefore $\cD$ and $\cD^1,...,\cD^p$ correspond to observational distribution $\bbP_{\hat{U}}$ and (hard) interventional distributions $\bbP_{\hat{U}}^{\{\pi(1)\}},...,\bbP_{\hat{U}}^{\{\pi(p)\}}$. We thus have full identifiability of $\cG_{\pi}$ (using results in \cite{hauser2012characterization}). Step 2 is proven.
\end{quote}

Combining the two steps, we have shown that $\langle U, \cG, I_1,...,I_p\rangle$ can be identified up to its $\cM$-equivalence class.
\end{proof}


\subsection{Unknown Latent Dimension}

The former section assumes that the dimension $p$ of latent causal variable $U$ is known. However, this might be impossible in many applications, where the goal of representation learning involves finding the number of causal variables. It turns out we can generalize the proof to unknown $p$. We make the following remark before the proof.

\begin{remark}
The condition in Corollary~\ref{cor:1} of having interventional data $\cD^1,...,\cD^{K}$ from at least one hard intervention on each latent node are available assumes we know an upper bound $K\geq p$ of the ground-truth latent dimension $p$. It does not however assume that we know which ones of $\cD^1,...,\cD^{K}$ correspond to intervening the same latent node. 
\end{remark}
% The following corollary shows that identifiability still holds if we only have an upper bound of the ground-truth latent dimension $p$.

% \begin{corollary}\label{cor:2}
%     Suppose Assumption \ref{assumption:1} holds true and observational data $\cD$ and interventional data $\cD^1,...,\cD^{p'}$ from at least one hard intervention on each latent node are available, where each intervention preserves support with non-empty interior on all variables aside from its intervention target. Then $\langle U,\cG,I_1,...,I_{p'}\rangle$ are identifiable up to its $\cM$-equivalence class.
% \end{corollary}

\begin{proof}[Proof of Corollary \ref{cor:1}]
    The proof is similar to the case where $K=p$. However, in step 1, we also identify the latent dimension $p$ and which ones of $\cD^1,...,\cD^{K}$ correspond to intervening the same latent node.

    \textbf{Step 1:} we solve for the smallest integer $\hat{p}\leq K$ and a mapping $\hat{g}:\bbR^n\rightarrow\bbR^{\hat{p}}$ that satisfy three conditions: (1) there exists a full row rank polynomial $\hat{f}(\cdot)$ such that $\hat{f}\circ\hat{g}(X)=X$ for all $X\in\cD\cup\cD^1\cup...\cup \cD^{K}$; (2) for each $i\in[\hat{p}]$, there exists $\hat{i}\in[K]$ such that $\hat{g}(X)_i$ is a constant for all $X\in\cD^{\hat{i}}$.

    Denote $\hat{U}=\hat{g}(X)\in\bbR^{\hat{p}}$. Using similar arguments as the case where $K=p$, we have that there exist two polynomials such that $\hat{U}=poly_1(U)$ and $U=poly_2(\hat{U})$ for all $U\in\bbU$ and $\hat{U}\in\hat{g}(\bbX)$. Since $\bbU$ has a non-empty interior, the dimension of $\hat{U}$ can not be smaller than the dimension of $U$, i.e., $\hat{p}\geq p$. Since there exists a solution to conditions (1) and (2) when $\hat{p}=p$. Therefore solving for conditions (1) and (2) with the smallest $\hat{p}$ gives $\hat{p}=p$ and $\hat{U}=U\Lambda+B$ for some non-singular matrix $\Lambda$ and vector $B$. Then, following similar proofs in the case where $K=p$, we can use condition (2) to show that $\Lambda$ is diagonal. In addition, we can also identify the intervention targets of $\langle I_{\hat{1}},...,I_{\hat{p}}\rangle$ up to its $\cM$-equivalence class. Then for each $\cD^i$ of $\cD^1,...,\cD^K$, we can check which dimension of $\hat{g}(\cD^i)$ collapses to one value and match its intervention target to one of $I_{\hat{1}},...,I_{\hat{p}}$. This then gives us the identifiability of intervention targets $\langle I_{1},...,I_{K}\rangle$ up to its $\cM$-equivalence class.

    \textbf{Step 2} is the same as the proof of Corollary \ref{cor:1}, where we can identify $\cG$ up a permutation that is consistent with that of $U,I_1,...,I_{K}$. Therefore we can identify $\langle U,\cG,I_1,...,I_{K}\rangle$ up to its $\cM$-equivalence class.
\end{proof}


\begin{remark}\label{rmk:1}
This proof indicates we can identify $\langle U,\cG,I_1,...,I_K\rangle$ up to $\cM$-equivalence class by solving for the smallest integer $\hat{p}\leq K$ and an encoder $\hat{g}:\bbR^n\rightarrow\bbR^{\hat{p}}$ that satisfies (1) there exists a full row rank polynomial decoder $\hat{f}(\cdot)$ such that $\hat{f}\circ \hat{g}(X)=X$ for all $X\in \cD\cup\cD^1\cup ...\cup\cD^K$, and (2) for each $i\in [\hat{p}]$, there exists $\hat{i}\in[K]$ such that $\hat{g}(X)_i$, the $i$-th entry of $\hat{g}(X)$, is a constant for all $X\in\cD^{\hat{i}}$. In Appendix \ref{app:d}, we will use this observation to show that our discrepancy-based VAE is consistent in the limit of infinite data. 
\end{remark}

\begin{remark}\label{rmk:2}
Suppose by solving $\hat{g}$ in Remark~\ref{rmk:1}, we identify $\langle\hat{U},\hat{\cG},\hat{I}_1,...,\hat{I}_K\rangle$ such that $\hat{U}_{\pi(i)}:=\hat{g}(X)_{\pi(i)}=\lambda_i f^{-1}(X)_i+b_i =\lambda_i U_i+b_i$, $\hat{\cG}=\cG_{\pi}$, and $\hat{I}_k=\pi(I_k)$ for all $k\in[K]$. The proof of Theorem~\ref{thm:1} also shows (with slight extensions) that (1) for all $k\in[K]$ with $i\in I_k$, the constant $\hat{a}_{\pi(i)}:=\hat{U}_{\pi(i)}=\hat{g}(X)_{\pi(i)}$ for $X\in \cD^{k}$ satisfies $\hat{a}_{\pi(i)}=\lambda_i a_i+b_i$, where $a_i$ is the fixed value to which the hard intervention $I_{k}$ has set $U_{i}$; (2) the decoder $\hat{f}=f\circ M_{\Lambda,B}^{-1}\circ M_{\pi}$, where $\big(M_{\pi}^{-1}\circ M_{\Lambda,B}(U)\big)_{\pi(i)}=\lambda_iU_i+b_i$. 
\end{remark}



==> content/old/append-b.tex <==
\section{Proof of Identifiability with Soft Interventions}\label{app:b}

Note that the proof for hard interventions can be derived by examining the support of the learned variables $U$ from observational and interventional samples $X$. This is provided by the fact that a hard intervention reduces the support of its intervention target to a single focal point. For shift interventions, however, the support of the intervention target can stay the same. In this case, we need to look at finer-grained information, such as the probability masses. 

\subsection{Assumptions}

We have shown in Example \ref{exp:3} that it is possible to have reversed directions between the intervention targets of $\cD^1,...,\cD^K$ without further assumptions. In the case of Example \ref{exp:3}, the alternative latent variable $\hat{U}_2 = U_2-U_1$ does not depend on $U_1$. This means that it has the same marginal distribution induced by $\bbP_U$ and $\bbP_U^{\{1\}}$. Therefore we can construct a latent DAG where $\hat{U}_2$ is upstream of $\hat{U}_1$ and $I_1=\{1\}$ is an intervention on $\hat{U}_1$, creating a reversed edge. To avoid such cases, we make the following faithfulness assumption.

\begin{assumption}\label{ass:faithfulness} 
    We assume that $\bbP_{U}$ is faithful to $\cG$ (c.f. \cite{uhler2013geometry}). Furthermore, we assume that $\bbP_{U}^{I_1},...,\bbP_{U}^{I_K}$ satisfy the following \textit{linear faithfulness} with respect to $\cG$: for any subset $\mathcal{I}$ containing $p$ elements of $\{I_1,...,I_K\}$ whose intervention targets span $[p]$, it satisfies for every node $j$ in $\cG$ with $\an_{\cG}(j)\neq\varnothing$ and all $c_i\in \bbR$ for $i\in\an_{\cG}(j)$\footnote{$\an_{\cG}(j)$ denotes the ancestors of $j$ (i.e., all nodes that have a directed path points to $j$).}
    \begin{align*}
    \bbP_U^{I} \big( U_j+\sum_{i\in\an_{\cG}(j)} c_i U_i \big)
    & \neq 
    \bbP_U \big( U_i+ \sum_{i\in\an_{\cG}(j)} c_i U_i \big)
    \end{align*}
    for some $I\in\mathcal{I}$ that targets some node in $\an_{\cG}(j)$. Moreover, $\bbP_U^{I} \big(U_j+c_i U_i \big)\neq \bbP_U \big( U_i+ c_i U_i \big)$ for all $i\in \an_{\cG}(j)$ and $I\in\mathcal{I}$ where $I$ targets node $i$.
\end{assumption}

Note that when all $c_i=0$, $\bbP^{I_k}_U(U_j)\neq \bbP_U(U_j)$ for ancestor $U_i$ of $U_j$ and $I_k$ targeting $i$ is a weaker form of the interventional faithfulness proposed in \cite{yang2018characterizing}. In fact, the following lemma shows that linear faithfulness can be reduced to a finite number of inequality constraints. Thus Assumption \ref{ass:faithfulness} holds almost surely \cite{uhler2013geometry}.\todo{am i citing the right paper here?}

\begin{lemma}\label{lm:lf}
  $\bbP_{U}^{I_1},...,\bbP_{U}^{I_K}$ satisfy the linear faithfulness assumption with respect to $\cG$ if and only if: for any subset $\mathcal{I}$ containing $p$ elements of $\{I_1,...,I_K\}$ whose intervention targets span $[p]$, it satisfies
  \begin{itemize}
      \item[(i)] for each node $j\in \cG$ with $\an_{\cG}(j)\neq\varnothing$, there exists some $I\in\mathcal{I}$ such that $I$ targets some node in $\an_{\cG}(j)$ and 
   \begin{equation}\label{eq:lm-lf}
    \bbP_U^{I} \big( U_j+\sum_{i\in\an_{\cG}(j)} C_i U_i \big)
    \neq 
    \bbP_U \big( U_i+ \sum_{i\in\an_{\cG}(j)} C_i U_i \big),
   \end{equation}
    where $C_i\in \bbR$~~for $i\in\an_{\cG}(j)$ is defined recursively as 
    \begin{equation}\label{eq:lm-lf2}
    C_i=-\frac{\bbE_{\bbP_U}(U_j+\sum_{l\in \an_{\cG}(j)\cap\de_{\cG}(i)}C_lU_l)-\bbE_{\bbP_U^{\{i\}}}(U_j+\sum_{l\in \an_{\cG}(j)\cap\de_{\cG}(i)}C_lU_l)}{\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{\{i\}}}(U_i)},
    \end{equation}
    where $\{i\}$ is the intervention amongst $\mathcal{I}$ that targets node $i$;
    \item[(ii)] for all $i\in\an_{\cG}(j)$, there is
    \begin{equation}\label{eq:lm-lf0}
    \bbP_U^{\{i\}}(U_j+C_i'U_i)\neq \bbP_U(U_j+C_i'U_i)
    \end{equation}
    for $C_i'=-\nicefrac{\big(\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{\{i\}}}(U_j)\big)}{\big(\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{\{i\}}}(U_i)\big)}$. Here $\de_{\cG}(i)$ denotes the descendants of $i$ in $\cG$ (i.e., all nodes that lie on some directed path from $i$). ${\{i\}}$ is defined the same as above. 
  \end{itemize}
\end{lemma}

\begin{proof}
    First, we show that Eq.~\eqref{eq:lm-lf2} has a unique solution. Note that by definition $\bbE_{\bbP_U}(U_i)\neq\bbE_{\bbP_U^{\{i\}}}(U_i)$, and therefore the quantity on the right hand side of Eq.~\eqref{eq:lm-lf2} is well defined. To see that it has a unique solution, we solve for $C_i$ iteratively based on the number of nodes in $\an_{\cG}(j)\cap\de_{\cG}(i)$: when $|\an_{\cG}(j)\cap\de_{\cG}(i)|=0$, $C_i$ are directly given by $-\nicefrac{\big(\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{\{i\}}}(U_j)\big)}{\big(\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{\{i\}}}(U_i)\big)}$. Then when $|\an_{\cG}(j)\cap\de_{\cG}(i)|=1$, we can solve $C_i$ based on $C_{i'}$ with $|\an_{\cG}(j)\cap\de_{\cG}(i)|=0$. These will then give us a unique solution.


    Next, we show that Eq.~\eqref{eq:lm-lf} implies for all $c_i\in \bbR$, there is
    \begin{equation}\label{eq:lm-lf3}
    \bbP_U^{I} \big( U_j+\sum_{i\in\an_{\cG}(j)} c_i U_i \big)\neq \bbP_U \big( U_i+ \sum_{i\in\an_{\cG}(j)} c_i U_i \big),
    \end{equation}
    for some $I\in\mathcal{I}$ such that $I$ targets some node in $\an_{\cG}(j)$. If $c_i=C_i$ for all $i\in \an_{\cG}(j)$, then Eq.~\eqref{eq:lm-lf2} holds true directly by Eq.~\eqref{eq:lm-lf}. If $c_i\neq C_i$ for some $i\in \an_{\cG}(j)$, let $i'$ be the most downstream node amongst $\an_{\cG}(j)$ such that $c_{i'} \neq C_{i'}$. In other words, there is no $i\in\an_{\cG}(j)\cap\de_{\cG}(i')$ with $c_{i} \neq C_{i}$, where $i\in\de_{\cG}(i')$ if and only $i'\in \an_{\cG}(i)$. Note that $\bbP_U^{\{i'\}}$ does not change the distribution of $U_i$ for $i\notin \de_{\cG}(i')$. By linearity of expectations, we have 
    \begin{align*}
        & \bbE_{\bbP_U}\big( U_j+\sum_{i\in\an_{\cG}(j)} c_i U_i \big)-\bbE_{\bbP_U^{\{i'\}}}\big( U_j+\sum_{i\in\an_{\cG}(j)} c_i U_i \big) \\
        % ={}& \bbE_{\bbP_U}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} c_i U_i \big) - \bbE_{\bbP_U^{\{i'\}}}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} c_i U_i \big) + c_{i'}\big(\bbE_{\bbP_U}(U_{i'})-\bbE_{\bbP_U^{\{i'\}}}(U_{i'})\big)  \\
        ={} & \bbE_{\bbP_U}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} C_i U_i \big) - \bbE_{\bbP_U^{\{i'\}}}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} C_i U_i \big) + c_{i'}\big(\bbE_{\bbP_U}(U_{i'})-\bbE_{\bbP_U^{\{i'\}}}(U_{i'})\big)\\
        \neq{}& \bbE_{\bbP_U}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} C_i U_i \big) - \bbE_{\bbP_U^{\{i'\}}}\big(U_j+\sum_{i\in\an_{\cG}(j)\cap\de_{\cG}(i)} C_i U_i \big) + C_{i'}\big(\bbE_{\bbP_U}(U_{i'})-\bbE_{\bbP_U^{\{i'\}}}(U_{i'})\big) = 0.
    \end{align*}
    Therefore Eq.~\eqref{eq:lm-lf3} is satisfied for $I\in\mathcal{I}$ targeting $i'$.

    Finally, we show that Eq.~\eqref{eq:lm-lf0} implies for all $c_i\in \bbR$, there is $\bbP_U^{\{i\}}(U_j+c_iU_i)\neq \bbP_U(U_j+c_iU_i)$. If $c_i=C_i'$, this is proven directly by Eq.~\eqref{eq:lm-lf0}. If $c_i\neq C_i'$, then $\bbE_{\bbP_U}(U_j+c_iU_i)-\bbE_{\bbP_U^{\{i\}}}(U_j+c_iU_i)\neq \bbE_{\bbP_U}(U_j+C_i'U_i)-\bbE_{\bbP_U^{\{i'\}}}(U_j+C_i'U_i)=0$. Therefore there is always $\bbP_U^{\{i\}}(U_j+c_iU_i)\neq \bbP_U(U_j+c_iU_i)$. We thereby proved linear faithfulness is satisfied if Eq.~\eqref{eq:lm-lf} and Eq.~\eqref{eq:lm-lf0} hold true for every node $j\in\cG$. 
\end{proof}

% Furthermore, we can show that Assumption~\ref{ass:faithfulness} holds if the causal mechanisms are strictly convex and $I_1,...,I_K$ include two different shift interventions per latent node.

% \begin{corollary}\label{corr:lmlf}
%     Suppose for all $i\in\cG$ and $j\in\an_{\cG}(i)$, the conditional expectation $\bbE_{\bbP_{U}}(U_j|U_i)$ is strictly convex in $U_i$. If $I_1,...,I_K$ include two different shift interventions per latent node, then Assumption \ref{ass:faithfulness} always holds.
% \end{corollary}

% \begin{proof}
%     We only need to show that $\bbP_{U}^{I_1},...,\bbP_{U}^{I_K}$ satisfy (i) and (ii) in Lemma~\ref{lm:lf}. To see (i), let $I_k$ be the intervention targeting the most downstream parent $i$ of $j$ (if there exists multiple, take an arbitrary one). Then $\bbP^{I_k}(U_j+cU_i)=\bbP(U_j+cU_i)$ only if for one value of $c=-\nicefrac{\big(\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{I_k}}(U_j)\big)}{\big(\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{I_k}}(U_i)\big)}$. 

%     Let $I_{k'}$ be the other shift intervention that targets $i$. Assume $I_k,I_{k'}$ correspond to shift values $a,b$ respectively. Without loss of generality, assume $a>b$. Denote $\bbE_{\bbP_U}(U_j|U_i)=m(U_i)$. Then by the law of expectation,
%     \begin{align*}
%     \frac{\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{I_k}}(U_j)}{\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{I_k}}(U_i)} & = \bbE_{\bbP_{U}}\left(\frac{m(U_i)-m(U_i+a)}{a}\right), \\
%     \frac{\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{I_{k'}}}(U_j)}{\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{I_{k'}}}(U_i)} & = \bbE_{\bbP_{U}}\left(\frac{m(U_i)-m(U_i+b)}{b}\right).
%     \end{align*}
%     Since $m$ is strictly convex, $\nicefrac{m(U_i)-m(U_i+a)}{a}\leq \frac{m(U_i)-m(U_i+b)}{b}$.
% \end{proof}
% \newpage

\begin{remark}
    Note that linear structural equation models will not satisfy linear faithfulness. To see this, consider the most upstream $i\rightarrow j\in \cG$ (i.e., $i$ has no parents and $i$ has no children that point to $j$). When $C_i=-\nicefrac{\big(\bbE_{\bbP_U}(U_j)-\bbE_{\bbP_U^{\{i\}}}(U_j)\big)}{\big(\bbE_{\bbP_U}(U_i)-\bbE_{\bbP_U^{\{i\}}}(U_i)\big)}$, $-C_i$ equals to the coefficient of $U_i$ in $U_j$. Therefore, variable $U_j+C_iU_i$ is independent of $U_i$ and its distribution will not change if we shift $U_i$. However, in section \ref{sec:VAE}, we still illustrate our VAE framework using a linear structural equation for the purpose of simplicity. In Appendix \ref{app:d}, we will discuss the implication of these constraints on the consistency of the proposed discrepancy-based VAE.
\end{remark}

Under Assumption \ref{ass:faithfulness}, even without any reversed edges, Example \ref{exp:2} indicates that there can still be missing or excessive edges. The example stems from the fact that we can easily remove (or add) the edge between $1\rightarrow 3$ by merging (or separating) the effect of $U_1$ on $U_3$ through $U_2$. We make the following assumption to avoid such cases. To state the assumption, we define, for an edge $i\rightarrow j\in \cG$, $\dpa_{\cG}(i,j)=\de_{\cG}(i)\cap \pa_{\cG}(j)$ to be the set of nodes in $\cG$ that are both descendants of $i$ and parents of $j$. Note that $\dpa_{\cG}(i,j)$ does not include $j$. Intuitively, $\dpa_{\cG}(i,j)$ is the parents of $j$ that lie in between $i$ and $j$. Figure \ref{fig:a0} illustrates $\dpa_{\cG}(i,j)$ for Example \ref{exp:2} with $i=1$ and $j=3$. 

\begin{figure}[h!]
     \centering
     \includegraphics[width=.15\textwidth]{fig/fig-a0.png}
     \vspace{-.1in}
     \caption{An example of $\dpa_{\cG}(i,j)$ in a 3-node DAG. Red edge: $i=1$ and $j=3$. Purple node: $\dpa_{\cG}(i,j)$.}
     \label{fig:a0}
\end{figure}

\begin{assumption}\label{ass:3} 
    We assume for every edge $i\rightarrow j\in\cG$, there do \textit{not} exist $c_j,c_k\in \bbR$ for $k\in \dpa_{\cG}(i,j)$ such that $U_i$ and $U_j+c_jU_i$ are conditionally independent given $\{U_k+c_kU_i\}_{k\in  \dpa_{\cG}(i,j)}$ and $\{U_k\}_{k\in  \pa_{\cG}(j) \setminus (\{i\}\cup \dpa_{\cG}(i,j))}$.
\end{assumption}

Intuitively, this assumption ensures that we will not miss any edge $i\rightarrow j$ by merging the effect of $U_i$ to $U_j$ into nodes that lie between them.
Note that when $c_j=c_k=0$ for $k\in \dpa_{\cG}(i,j)$, variables $\{U_k\}_{k\in  \dpa_{\cG}(i,j)}$ and $\{U_k\}_{k\in  \pa_{\cG}(j) \setminus (\{i\}\cup \dpa_{\cG}(i,j))}$ constitute $\{U_k\}_{k\in  \pa_{\cG}(j) \setminus \{i\}}$. In this case, $U_i$ and $U_j$ are \textit{not} conditionally independent given $\{U_k\}_{k\in  \pa_{\cG}(j) \setminus \{i\}}$ by the faithfulness of $\bbP_U$. In fact, this assumption is closely related to the linear faithfulness in Assumption \ref{ass:faithfulness}, shown in the following lemma.
% does this hold true for general graphs? no, consider u_3=(u_1+u_2)^2. this is only true by assuming some minimality of the graph, e.g., in trees, the minimality is that each node has only one parent

\begin{lemma}
If $\cG$ is a tree graph and Assumption \ref{ass:faithfulness} holds for some $I_1,...,I_K$, then Assumption \ref{ass:3} holds.
\end{lemma}

\begin{proof}
    Suppose $\cG$ is a tree graph and Assumption \ref{ass:faithfulness} holds. For any edge $i\rightarrow j\in\cG$, since $j$ only has one parent $i$, we only need to show that $U_i$ and $U_j+c_jU_i$ are not conditionally independent for any $c_j\in \bbR$.

    For $c_j=0$, $U_i$ and $U_j$ are not conditionally independent by the faithfulness of $\bbP_U$. For $c_j\neq 0$, suppose $U_i$ and $U_j+c_jU_i$ are conditionally independent. Then for any $l,r\in \bbR$,
    \begin{align*}
        \bbP_{U}(U_j+c_jU_i=l) & = \bbP_{U}(U_j+c_jU_i=l|U_i=r) \\
        & = \bbP_{U}(U_j=l-c_jr|U_i=r).
    \end{align*}
    Since this is true for any $r\in\bbR$, we have for any $k\in [p]$
    \begin{align*}
        \bbP_{U}(U_j+c_jU_i=l) & = \int \bbP_{U}(U_j=l-c_jr|U_i=r)\cdot\bbP_{U}^{I_k}(U_i=r)dr.
    \end{align*}
    Note that $\bbP_{U}(U_j|U_i)=\bbP_{U}^{I_k}(U_j|U_i)$ for all $I_k$ targeting nodes in $\an_{\cG}(j)$, we thus have 
    \begin{align*}
        \bbP_{U}(U_j+c_jU_i=l) & = \int \bbP_{U}^{\{i\}}(U_j=l-c_jr|U_i=r)\cdot\bbP_{U}^{I_k}(U_i=r)dr\\
        & = \int \bbP_{U}^{I_k}(U_j=l-c_jr,U_i=r) dr \\
        & =  \bbP_{U}^{I_k}(U_j+c_jU_i=l).
    \end{align*}
    A contradiction to linear faithfulness in Assumption \ref{ass:faithfulness}. Therefore $U_i$ and $U_j+c_jU_i$ are not conditionally independent.
\end{proof}

\subsection{Known Latent Dimension}

Similar to the case for hard interventions, we first consider an easier setting where the dimension $p$ of the latent causal variable $U$ is known and we have data from exactly one shift intervention per latent node, i.e., $K = p$ in Theorem~\ref{thm:1}. We will generalize the discussion to unknown
$p$ in the next section. We prove a useful lemma below.

\begin{lemma}\label{lm:a2}
    If random variables $A,B,C,D$ satisfy both $A\CI B|C,D$ and $A\CI C|B,D$, then $A\CI B|D$. Here $A\CI B|C,D$ denotes that $A$ and $B$ are conditionally independent given $C,D$; $A\CI C|B,D$ and $A\CI B|D$ are similarly defined.
\end{lemma}

\begin{proof}
    Since $A\CI B|C,D$, we have $\bbP(A|B=b,C=c,D)=\bbP(A|C=c,D)$ for any realizations $b$ of $B$ and $c$ of $C$. Similarly, we have $\bbP(A|B=b,C=c,D)=\bbP(A|B=b,D)$ by $A\CI C|B,D$. Thus for fixed $b$, there is $\bbP(A|B=b,D)=\bbP(A|C=c,D)$ for any realization $c$. Then $\bbP(A|B=b,D)=\int \bbP(A|C=c,D)\bbP(C=c|D)dc=\bbP(A|D)$. Since this is true for any $b$, we, therefore, have $A\CI B|D$.
\end{proof}




\begin{proof}[Proof of Theorem \ref{thm:1} ($K=p$)]

We show $\langle \cG,I_1,...,I_p\rangle$ is identifiable up to $\cM$-equivalence class by two steps: (Step 1) we first show that $U$ can be identified up to a linear transformation using a constrained matrix, (Step 2) we then show that $\langle \cG,I_1,...,I_p\rangle$ can be identified up to $\cM$-equivalence. 

In the first step, we construct two conditions that lead to a solution that recovers $U$ up to the allowed transformations. In the second step, we show that each solution to the first step leads to a DAG and the sparsest DAG corresponds to $\langle \hat{\cG},\hat{I}_1,...,\hat{I}_p\rangle$ that is  $\cM$-equivalent to the ground truth $\langle \cG,I_1,...,I_p\rangle$.


\textbf{Step 1:} we show that $U$ can be recovered up a linear transformation using a constrained (details to be defined below) matrix. This is achieved by solving a mapping $\hat{g}:\bbR^n\rightarrow \bbR^p$ that satisfies three conditions: 
%
(1) there exists a full row rank polynomial $\hat{f}(\cdot)$ such that $\hat{f}\circ\hat{g}(X)=X$ for all $X\in \cD\cup\cD^1\cup ...\cup\cD^p$;
%
(2) there exists a permutation $\rho$ of $[p]$ such that for each $i\in [p]$, comparing the marginal distributions of $\hat{g}(X)_i$ from $X\in \cD$ to $X\in\cD^j$, they differ for $j=\rho(i)$ and can only differ for $j\in\{\rho(1),...,\rho(i)\}$; 
%
(3) for the permutation $\rho$ in (2), there do not exist $i'<i\in [p]$ and $c\neq 0$, where $\hat{g}(X)_i$ has different marginal distributions from $X\in \cD$ to $X\in\cD^{\rho(i')}$ but $\hat{g}(X)_i-c\hat{g}(X)_{i'}$ has the same marginal distribution from $X\in \cD$ to $X\in\cD^{\rho(i')}$.

\begin{quote}
\textit{Proof of Step 1:}
First of all, there exists a solution by $\hat{g}=M_{\tau}\circ f^{-1}$, where $f$ is ground-truth mapping (it is invertible based Assumption \ref{assumption:1}.2) and $M_{\tau}$ is a permutation operation such that $M_{\tau}(V)=(V_{\tau(1)},...,V_{\tau(p)})$ for all $V\in \bbR^p$. Here $\tau$ is the ground-truth topological order of $\cG$ (if there are multiple, take an arbitrary one), i.e., $\tau(i)\rightarrow \tau(j)\in \cG$ only if $i<j$. 

To see that $\hat{g}$ satisfies condition (1): set $\hat{f}=f\circ M_\tau^{-1}$, then $\hat{f}\circ \hat{g}(X)=f\circ M_\tau^{-1}\circ M_{\tau}\circ f^{-1} (X)=X$. To see that $\hat{g}$ satisfies condition (2): let $\rho$ is a permutation of $[p]$ such that $\cD^{\rho(j)}$ corresponds to a shift intervention on $U_{\tau(j)}$, we have $\hat{g}(X)_i=(M_\tau\circ f^{-1}(X))_i=f^{-1}(X)_{\tau(i)}=U_{\tau(i)}$ which has different marginal distributions from $X\in\cD$ to $X\in\cD^j$ if $j=\rho(i)$. Moreover, they can only differ if $j\in\{\rho(1),...,\rho(i)\}$, since $j\in\{\rho(i+1),...,\rho(p)\}$ correspond to shifting $U_{\tau(i+1)},...,U_{\tau(p)}$ whom are not upstream of $U_{\tau(i)}$. To see that $\hat{g}$ and the defined $\rho$ above satisfies condition (3): for any $i'<i\in [p]$, $\hat{g}(X)_i=U_{\tau(i)}$ will only have a changed marginal under $\cD^{\rho(i')}$ as compared to $\cD$ if $\cD^{\rho(i')}$ corresponds to shifting an ancestor of $U_{\tau(i)}$. By the definition of $\rho$, $\cD^{\rho(i')}$ corresponds to a shift on $U_{\tau(i')}$. Therefore whenever $\hat{g}(X)_i=U_{\tau(i)}$ has a changed marginal under $\cD^{\rho(i')}$ as compared to $\cD$, it means $\tau(i')\in \an_{\cG}(i)$. By Assumption \ref{ass:faithfulness},~~$\hat{g}(X)_i-c\hat{g}(X)_{i'}=U_{\tau(i)}-cU_{\tau(i')}$ will always have different marginal distributions in $X\in \cD$ and $X\in \cD^{\rho(i')}$. Therefore $\hat{g}=M_{\tau}\circ f^{-1}$ is a solution to conditions (1), (2), and (3). 


Now let $\hat{g}$ be a solution to conditions (1), (2), and (3). Denote $\hat{U}=\hat{g}(X)$. Similar to the proof for Corollary \ref{cor:1}, any $\hat{g}$ that satisfies condition (1) must give $\hat{U}=U\Lambda+B$ for some non-singular matrix $\Lambda$ and vector $B$. We will show that $\Lambda$ is lower triangular up to a row permutation that is consistent with the ground-truth topological order.

Consider $\hat{U}_1=U\Lambda_{:,1}+B_1$. By condition (2), its marginal distribution is only allowed to change in one interventional distribution $\cD^{\rho(1)}$ as compared to the observational distribution. This means shifting $p-1$ nodes of $\cG$ will not change its marginal distribution. If $\Lambda_{:,1}$ has non-zero entries, let $j$ be the entry corresponding to the two most downstream node of $\cG$ amongst the nonzero entries. Then shifting $U_j$ will result in a change of the marginal distribution of $U\Lambda_{:,1}$, since it will shift the mean $U\Lambda_{:,1}$ by the amount of shift on $U_j$ times $\Lambda_{j,1}$. In addition, if $\an_{\cG}(j)\neq\varnothing$, then by Assumption \ref{ass:faithfulness}, shifting some node in $\an_{\cG}(j)$ will also result in a change of the marginal distribution of $U\Lambda_{:,1}$. Therefore $U\Lambda_{:,1}$ must equal to $\lambda_{\tau(1),1}U_{\tau(1)}$ for a source node\footnote{$j$ is a source node of $\cG$ if and only of $\pa_{\cG}(j)=\varnothing$.} $\tau(1)$ of $\cG$. Since the marginal distribution of $\hat{U}_1=\lambda_{\tau(1),1}U_{\tau(1)}+B_1$ changed from $\cD$ to $\cD^{\rho(1)}$, we must have $\lambda_{\tau(1),1}\neq 0$ and $\cD^{\rho(1)}$ must correspond to shifting $U_{\tau(1)}$, i.e, the source node $\tau(1)$ of $\cG$.

Next consider $\hat{U}_2=U\Lambda_{:,2}+B_2$. By condition (2), its marginal is only allowed to change\footnote{For brevity, we will use ``change" to mean ``change as compared to the observational distribution $\cD$''.} in $\cD^{\rho(1)}$ and $\cD^{\rho(2)}$. This means shifting $p-2$ nodes of $\cG$ will not change its marginal distribution. In addition, we know that $\cD^{\rho(1)}$ corresponds to shifting the source node ${\tau(1)}$. Consider the subgraph of $\cG$ after removing node $\tau(1)$. Consider $\hat{U}_2-\lambda_{\tau(1),2}\hat{U}_1$, where $\lambda_{\tau(1),2}\in\bbR$ is such that the coefficient of $U_{\tau(1)}$ is zero in $\hat{U}_2-\lambda_{\tau(1),2}\hat{U}_1$. Using similar arguments as above (with the subgraph of $\cG$ after removing node $\tau(1)$), we have that $\hat{U}_2-\lambda_{\tau(1),2}\hat{U}_1$ must equal to $\lambda_{\tau(2),2}U_{\tau(2)}$, where $\tau(2)$ is a source node of the subgraph of $\cG$ after removing node $\tau(1)$. In addition, since the marginal distribution of $\hat{U}_2=\lambda_{\tau(1),2}U_{\tau(1)}+\lambda_{\tau(2),2}U_{\tau(2)}+B_2$ changed from $\cD$ to $\cD^{\rho(2)}$ and the marginal of $\lambda_{\tau(1),2}U_{\tau(1)}$ stayed the same from $\cD$ to $\cD^{\rho(2)}$, it means $\lambda_{\tau(2),2}\neq 0$ and $\cD^{\rho(2)}$ corresponds to shifting $U_{\tau(2)}$, i.e., the source node $\tau(2)$ of the subgraph of $\cG$ after removing $\tau(1)$.

Following similar discussions for $\hat{U}_3,...,\hat{U}_p$. We have that for all $i\in [p]$, there is 
\begin{equation}\label{thm:eq-1}
 \hat{U}_i=\lambda_{\tau(1),i}U_{\tau(1)}+\lambda_{\tau(2),i}U_{\tau(2)}...+\lambda_{\tau(i),i}U_{\tau(i)}+B_i,
\end{equation}
where $\tau(i)$ is a source node of of the subgraph of $\cG$ after removing $\tau(1),...,\tau(i-1)$. In addition, $\lambda_{\tau(i),i}\neq 0$ and $\cD^{\rho(i)}$ corresponds to shifting $U_{\tau(i)}$.

Finally, we will use condition (3) to show that for $i'<i$ such that $\tau(i')\notin \an_{\cG}(\tau(i))$, there is always $\lambda_{\tau(i'),i}=0$. For any $i\in [p]$, if there exists $i'<i$ such that $\tau(i')\notin \an_{\cG}(\tau(i))$ and $\lambda_{\tau(i'),i}\neq 0$. Let $i'$ be the largest integer that satisfies $i'<i$, $\tau(i')\notin \an_{\cG}(\tau(i))$, and $\lambda_{\tau(i'),i}\neq 0$. Then for all $l$ such that $i'<l<i$ and $\tau(l)\in\de_{\cG}(\tau(i'))$, there is $\lambda_{\tau(l),i}=0$. Otherwise since $\tau(i')\notin \an_{\cG}(\tau(i))$, there is also $\tau(l)\notin \an_{\cG}(\tau(i))$. Therefore $l$ also satisfies $l<i$, $\tau(l)\notin \an_{\cG}(\tau(i))$, and $\lambda_{\tau(l),i}\neq 0$. A contradiction to $i'$ being the largest. Note also $\tau$ is the topological order, we thus have $U_{\tau(i')}$ corresponds to one of the most downstream nodes amongst all variables with nonzero coefficients in $\hat{U}_i$. Thus shifting $U_{\tau(i')}$ will shift the mean of $\hat{U}_i$ which results in a change of the marginal distribution of $\hat{U}_i$. Note that from results in the former paragraph, $\cD^{\rho(i')}$ corresponds to shifting $U_{\tau(i')}$. This means $\hat{U}_i$ has different marginal distributions from $\cD$ to $\cD^{\rho(i')}$. By condition (3), $\hat{U}_i-\lambda_{\tau(i'),i}\hat{U}_i'$ also has different marginal distributions from $\cD$ to $\cD^{\rho(i')}$. However, for any $l\in \de_{\cG}(\tau(i'))\cap\{i'\}$, the coefficient of $U_l$ in $\hat{U}_i-\lambda_{\tau(i'),i}\hat{U}_i'$ is zero. Thus the marginal distribution of $\hat{U}_i-\lambda_{\tau(i'),i}\hat{U}_i'$ will not change in $\cD^{\rho(i')}$. A contradiction. Therefore for $i'<i$ such that $\tau(i')\notin \an_{\cG}(\tau(i))$, there is always $\lambda_{\tau(i'),i}=0$. 


We can write $\hat{U}_i$ as Eq.~\eqref{thm:eq-1} where $\tau$ is the topological order and for $i'<i$ such that $\tau(i')\notin \an_{\cG}(\tau(i))$, there is always $\lambda_{\tau(i'),i}=0$. In addition, $\lambda_{\tau(i),i}\neq 0$ and $\cD^{\rho(i)}$ corresponds to shifting $U_{\tau(i)}$. Figure \ref{fig:a1} shows an example of such $\hat{U}$.
\end{quote}

\begin{figure}[t!]
     \centering
     \includegraphics[width=.4\textwidth]{fig/fig-a1.png}
     \vspace{-.1in}
     \caption{An example of the identified $\hat{U}$. Left: ground truth DAG structure. Right: an admissible solution $\hat{U}$.}
     \label{fig:a1}
\end{figure}

\textbf{Step 2:} let $\hat{U}$ be the variables returned by a solution $\hat{g}$ to conditions (1), (2), and (3) in the first step. Let $\rho$ be the permutation in condition (2) and $\tau$ be the permutation that satisfies Eq.~\eqref{thm:eq-1}. Note that the permutation $\tau$ is still unknown, but $\hat{U}$ and $\rho$ are revealed after solving $\hat{g}$. Let $\hat{\cG}$ be the sparsest DAG with nodes corresponding to $\hat{U}$ such that (a) it has topological order $1,2,...,p$, (b) it is an I-MAP (independence map, c.f., \cite{koller2009probabilistic})  of the distribution on $\hat{U}$ induced by $\hat{g}(\cD)$. We show that $\cG = \hat{\cG}_{\tau}$

\begin{quote}
\textit{Proof of Step 2:}
$\cG$ must be a subgraph of $\hat{\cG}_{\tau}$: if $\tau(i)\rightarrow \tau(j)\in \cG$, then there must be $\hat{U}_{i}\nCI\hat{U}_{j}|\hat{U}_{1},...,\hat{U}_{i-1},\hat{U}_{i+1},...,\hat{U}_{j-1}$. Otherwise assume $\hat{U}_{i}\CI\hat{U}_{j}|\hat{U}_{1},...,\hat{U}_{i-1},\hat{U}_{i+1},...,\hat{U}_{j-1}$, by the form in Eq.~\eqref{thm:eq-1}, we can retrieve $U_{\tau(1)},...,U_{\tau(i-1)}$ by linear transforming $\hat{U}_{1},...,\hat{U}_{i-1}$; this implies $U_{\tau(i)}\CI \hat{U}_{j}|U_{\tau(1)},...,U_{\tau(i-1)},\hat{U}_{i+1},...,\hat{U}_{j-1}$. By subtracting terms in $U_{\tau(1)},...,U_{\tau(i-1)}$ from $\hat{U}_{i+1},...,\hat{U}_{j}$ and then subtracting terms $\hat{U}_{l}$ from $\hat{U}_{l+1},...,\hat{U}_{j}$ for $l=i+1,...,j-1$ , we have that \begin{align*}
    U_{\tau(i)}\CI \lambda_{\tau(j),j}U_{\tau(j)}+c_jU_{\tau(i)}|&U_{\tau(1)},...,U_{\tau(i-1)},\\
    &\lambda_{\tau(i+1),i+1}U_{\tau(i+1)}+c_{i+1}U_{\tau(i)},...,\lambda_{\tau(j-1),j-1}{U}_{\tau(j-1)}+c_{j-1}U_{\tau(i)}
\end{align*}
for some $c_{i+1},...,c_j\in\bbR$. Moreover since $\lambda_{\tau(i_1),i_2}=0$ for all $i_1<i_2$ and $\tau(i_1)\notin \an_{\cG}(\tau(i_2))$, we have $c_{l}=0$ for any $l\notin\de_{\cG}(\tau(i))$. Since $\lambda_{\tau(i+1),i+1},...,\lambda_{\tau(j),j}$ are all nonzero, we can set $c_{i+1}',..., c_{j}'$ to be $\nicefrac{c_{i+1}}{\lambda_{\tau(i+1),i+1}},...,\nicefrac{c_{j}}{\lambda_{\tau(j),j}}$ respectively. Let $c_{1}'=...=c_{i-1}'=0$. Then $c_l'=0$ for any $l\notin \de_{\cG}(\tau(i))$ and the former conditional independence is equivalent to
\begin{equation}\label{thm1:s2-1}
\begin{aligned}
U_{\tau(i)}\CI U_{\tau(j)}+c_j'U_{\tau(i)}|&U_{\tau(1)}+c_1'U_{\tau(i)},...,U_{\tau(i-1)}+c_{i-1}'U_{\tau(i)}, \\
&U_{\tau(i+1)}+c_{i+1}'U_{\tau(i)},...,U_{\tau(j-1)}+c_{j-1}'U_{\tau(i)}.
\end{aligned}
\end{equation}
Since $\tau$ is a topological order of $\cG$, we have that $\{\tau(l)\}_{l\leq j-1}\cap\de_{\cG}(\tau(j))=\varnothing$ and $\pa_{\cG}(j)\subset \{\tau(l)\}_{l\leq j-1}$. Therefore, from the Markov property, we have
\[
U_{\tau(j)}\CI \{U_{\tau(l)}\}_{l\leq j-1, \tau(l)\notin\pa_{\cG}(\tau(j))} | \{U_{\tau(l)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))}.
\]
Since $\tau(i)\rightarrow\tau(j)\in\cG$, $U_{\tau(i)}$ is in $\{U_{\tau(l)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))}$ and we thus have
\begin{align}\label{thm1:s2-2}
U_{\tau(j)}+c_j'U_{\tau(i)}\CI \{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\leq j-1, \tau(l)\notin\pa_{\cG}(\tau(j))} |  U_{\tau(i)}, \{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))\setminus\{i\}}.
\end{align}
Let $A=U_{\tau(j)}+c_j'U_{\tau(i)}$, $B=U_{\tau(i)}$, $C=\{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\leq j-1, \tau(l)\notin\pa_{\cG}(\tau(j))}$ and $D=\{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))\setminus\{i\}}$, then by Eq.~\eqref{thm1:s2-1} and Eq.~\eqref{thm1:s2-2}, we can use Lemma \ref{lm:a2} to deduce 
\[
U_{\tau(i)}\CI U_{\tau(j)}+c_j'U_{\tau(i)}|\{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))\setminus\{i\}}.
\]
Since $c_l'=0$ for any $l\notin\de_{\cG}(\tau(i))$ and $\tau$ is the topological order, this can be further written as 
\[
U_{\tau(i)}\CI U_{\tau(j)}+c_j'U_{\tau(i)}|\{U_{\tau(l)}+c_l'U_{\tau(i)}\}_{l\in\dpa_{\cG}(i,j)}, \{U_{\tau(l)}\}_{l\leq j-1, \tau(l)\in\pa_{\cG}(\tau(j))\setminus(\{i\}\cup \dpa_{\cG}(i,j))}.
\]
A violation of Assumption \ref{ass:3}. Therefore there must be $\hat{U}_{i}\nCI\hat{U}_{j}|\hat{U}_{1},...,\hat{U}_{i-1},\hat{U}_{i+1},...,\hat{U}_{j-1}$. By (a) and (b), there must be an edge $i\rightarrow j\in\hat{\cG}$. Thus $\cG$ is always a subgraph of $\hat{\cG}_{\tau}$.

On the other hand if $\lambda_{\tau(i),j}=0$ for all $i<j$, by the faithfulness assumption (Assumption \ref{ass:faithfulness}), $\cG$ is an I-MAP of $U$, which means $\cG_{\tau^{-1}}$ is an I-MAP of $\hat{U}$ (here $\tau^{-1}$ is the permutation such that $M_{\tau^{-1}}\circ M_{\tau}$ is the identity). Since $\hat{\cG}$ is not sparser than $\cG_{\tau^{-1}}$, there must be $\hat{\cG}=\cG_{\tau^{-1}}$, i.e., $\hat{\cG}_\tau=\cG$. 
\end{quote}

Therefore by finding solution $\hat{g}$ that leads to $\hat{\cG}$ such that it has the minimum possible number of edges, we can recover $\cG$ up to an unknown permutation $\tau$ ($\cG=\hat{\cG}_{\tau}$, or equivalently, $\cG_{\tau^{-1}}=\hat{\cG}$). Moreover, suppose $\rho$ is the permutation that satisfies (2) for $\hat{g}$, by the arguments after Eq.~\eqref{thm:eq-1}, we know that $\cD^{\rho(i)}$ corresponds to intervening on node $\tau(i)$ of $\cG$, i.e., $I_{\rho(i)}=\{\tau(i)\}$. Let $\hat{I}_i=\{\rho^{-1}(i)\}$, noting that $\rho$ is revealed after solving $\hat{g}$. We have $\hat{I}_i=\tau^{-1}\circ\tau\circ\rho^{-1}(i)=\tau^{-1}(I_i)$. Denote $\pi=\tau^{-1}$. Then $\hat{\cG}=\cG_{\pi}$ and $\hat{I}_i=\pi(I_i)$ for all $i\in [p]$. Therefore we can identify $\langle\hat{\cG},\hat{I}_1,...,\hat{I}_p\rangle$ that are in the same $\cM$-equivalance class as $\langle\cG,I_1,...,I_p\rangle$.
\end{proof}


\subsection{Unknown Latent Dimension}

We extend the proof to the general setting of Theorem \ref{thm:1} where the dimension $p$ of latent $U$ is unknown and only an upper bound $K\geq p$ is known.
% \begin{corollary}\label{cor:3}
%     If Assumptions \ref{assumption:1},\ref{ass:faithfulness},\ref{ass:3} hold true and observational data $\cD$ and interventional data $\cD^1,...,\cD^{p'}$ from at least one shift intervention on each latent node are available, $\langle \cG,I_1,...,I_{p'}\rangle$ are identifiable up to its $\cM$-equivalence class.
% \end{corollary}

\begin{proof}[Proof of Theorem \ref{thm:1}]
    The proof is similar to a combination of Corollary \ref{cor:1} and Theorem \ref{thm:1} with $K=p$. In the first step, we identify both $p$ and $U$ up to the allowed transformation in the proof of the case where $K=p$.

    \textbf{Step 1:} we solve for the smallest integer $\hat{p}\leq K$ and a mapping $\hat{g}:\bbR^n\rightarrow \bbR^{\hat{p}}$ that satisfies four conditions: (1) there exists a full row rank polynomial $\hat{f}(\cdot)$ such that $\hat{f}\circ\hat{g}(X)=X$ for all $X\in\cD\cup\cD^1\cup...\cup\cD^{K}$; (2) there exists a subset of $\hat{p}$ elements $\rho_1,...,\rho_{\hat{p}}$ from $[K ]$ such that for each $i\in[\hat{p}]$, comparing the marginal distributions of $\hat{g}(X)_i$ from $X\in\cD$ to $X\in\cD^{j}$, they differ for $j=\rho_{i}$ and do not differ for $j=\rho_{i+1},...,\rho_{\hat{p}}$; (3) for the subset in (2), there do not exist $i'<i\in [\hat{p}]$ and $c\neq 0$, where $\hat{g}(X)_i$ has different marginal distributions from $X\in\cD$ to $X\in\cD^{\rho_{i'}}$ but $\hat{g}(X)_i-c\hat{g}(X)_{i'}$ has the same marginal distribution from $X\in\cD$ to $X\in \cD^{\rho_{i'}}$.

    Denote $\hat{U}=\hat{g}(X)\in\bbR^{\hat{p}}$. Using similar arguments as in the proof of Corollary \ref{cor:1}, we have $\hat{p}=p$ and $\hat{U}=U\Lambda +B$ for some non-singular matrix $\Lambda$ and vector $B$. Then, following similar arguments in the proof of Theorem \ref{thm:1} when $K=p$, we can use conditions (2) and (3) to write $\hat{U}_i$ as Eq.~\eqref{thm:eq-1} where $\tau$ is the topological order and for $i'<i$ such that $\tau(i')\notin\an_{\cG}(\tau(i))$, there is always $\lambda_{\tau(i'),i}=0$. In addition, $\lambda_{\tau(i),i}\neq 0$ and $\cD^{\rho_i}$ corresponds to shifting $U_{\tau(i)}$. 
    
    For $\cD^j$ where $j\notin\{\rho_1,...,\rho_p\}$, let $i\in[p]$ be the smallest such that $\hat{g}(X)_i$ has different marginal distributions from $X\in\cD$ to $X\in\cD^{j}$. Then $\cD^j$ corresponds to shifting $U_{\tau(i)}$. To see this, suppose $\cD^j$ corresponds to shifting $U_{\tau(i')}$. Since $\tau$ is the topological order, based on Eq.~\eqref{thm:eq-1}, $\hat{g}(X)_{i'}=\hat{U}_{i'}$ must have different marginal distributions from $X\in\cD$ to $X\in\cD^j$. Since $i$ is the smallest, we have $i\leq i'$. However by Eq.~\eqref{thm:eq-1}, $\hat{g}(X)_{i''}=\hat{U}_{i''}$ must have the same marginal distribution from $X\in\cD$ to $X\in\cD^j$ for any $i''<i'$. Therefore $i\geq i'$. Thus $i'=i$. Therefore we can also identify which ones of $\cD^1,...,\cD^{K}$ correspond to shifting the same latent node.

    \textbf{Step 2} is the same as the case where $K=p$. We can identify $\langle \cG,I_1,...,I_{K}\rangle$ up to its $\cM$-equivalence class by finding the solution $\hat{g}$ to step 1 that leads to the sparsest DAG.    
\end{proof}


\begin{remark}\label{rmk:5}
This proof indicates we can identify $\langle\cG,I_1,...,I_K\rangle$ up to $\cM$-equivalence class by solving for the smallest $\hat{p}$ and an encoder $\hat{g}:\bbR^n\rightarrow\bbR^{\hat{p}}$ that satisfies 
\begin{enumerate}
    \vspace{-.15in}
    \item[(1)] there exists a full row rank polynomial decoder $\hat{f}(\cdot)$ such that $\hat{f}\circ \hat{g}(X)=X$ for all $X\in \cD\cup\cD^1\cup ...\cup\cD^K$;
    \vspace{-.1in}
    \item[(2)] there exists a subset of $\hat{p}$ elements $\rho_1,...,\rho_{\hat{p}}$ from $[K ]$ such that for each $i\in[\hat{p}]$, comparing the marginal distributions of $\hat{g}(X)_i$ from $X\in\cD$ to $X\in\cD^{j}$, they differ for $j=\rho_{i}$ and do not differ for $j=\rho_{i+1},...,\rho_{\hat{p}}$;
    \vspace{-.1in}
    \item[(3)] for the subset in (2), there do not exist $i'<i\in [\hat{p}]$ and $c\neq 0$, where $\hat{g}(X)_i$ has different marginal distributions from $X\in\cD$ to $X\in\cD^{\rho_{i'}}$ but $\hat{g}(X)_i-c\hat{g}(X)_{i'}$ has the same marginal distribution from $X\in\cD$ to $X\in \cD^{\rho_{i'}}$;
    \vspace{-.1in}
    \item[(4)] DAG $\cG$ that is the sparsest I-MAP of $\hat{U}=\hat{g}(U)$ with topological order $1,2,...,\hat{p}$ has the minimum possible number of edges across all $\hat{g}$ that satisfies (1), (2), and (3).
    \vspace{-.15in}
\end{enumerate}
We will use this observation in Appendix \ref{app:d} to show that our discrepancy-based VAE is consistent in the limit of infinite data.
\end{remark}

\begin{remark}\label{rmk:6}
Suppose the solution $\hat{g}$ to Remark~\ref{rmk:5} recovers $\langle\hat{\cG},\hat{I}_1,...,\hat{I}_K\rangle$ such that $\hat{\cG}=\cG_{\pi}$ and $\hat{I}_k=\pi(I_k)$ for all $k\in [K]$.
% The proof for Theorem~\ref{thm:1} shows that by solving $\hat{g}$ in Remark~\ref{rmk:1}, we can identify $U$ up to $\hat{U}:=\hat{g}(X)= f^{-1}(X)\Lambda+B = U\Lambda+B$, where $\Lambda$ is a constrained matrix defined by Eq.~\eqref{thm:eq-1}. 
The proof for Theorem~\ref{thm:1} also shows (with slight extensions) that (1) for all $k\in[K]$ such that $i\in I_k$, the constant $\hat{a}_{\pi(i)}:=\bbE_{\cD^{k}}(\hat{U}_{\pi(i)})-\bbE_{\cD}(\hat{U}_{\pi(i)})=\bbE_{\cD^{k}}(\hat{g}(X)_{\pi(i)})-\bbE_{\cD}(\hat{g}(X)_{\pi(i)})$ satisfies $\hat{a}_{\pi(i)}=\lambda_{i,\pi(i)}a_{i}$, where $\Lambda$ the constrained matrix in Eq.~\eqref{thm:eq-1} and $a_{i}$ is the value that the intervention $I_k$ has shifted $U_{i}$; (2) the decoder $\hat{f}=f\circ M_{\Lambda,B}^{-1}$, where $M_{\Lambda,B}(U)=U\Lambda+B$. 
\end{remark}


==> content/old/discrepancy-vae-old.tex <==
\section{Discrepancy-based VAE Formulation}
\label{sec:VAE}


\begin{itemize}
    \item Having framed our identifiability guarantee using a combinatorial optimization program, we now transition our focus to developing a practical algorithm for causal disentanglement.

    \item Inspired by our characterization in (TODO: ref theorem), we develop a generative modeling approach.
    
    \item In particular, we develop a generative modeling approach. \cite{lopez2018deep,khemakhem2020variational,yang2021causalvae,lopez2022learning}

    \item Maximize penalized log-likelihood.

    \item Several approaches: exact search, greedy search, gradient-based search (citations).

    \item Take gradient-based approach, use autoencoding variational Bayes. \cite{lippe2022citris,lopez2022learning,brehmer2022weakly}

    \item Benefits: computational efficiency, ease of implementation, flexibility, e.g. incorporate inductive biases about the decoder

    \item In particular, fix a distribution over exogenous noise variables $Z$.

    \item We use these to generate latent causal variables $U$ using a causal graph + interventions.

    \item We train a decoder $\hatf$ to generate the observational samples.

    \item We train an encoder $p_\theta$ to approximately match the posterior $p(Z \mid X)$.

    \item Challenge: unpaired interventional datasets.

    \item Solution: add MMD loss using \textit{virtual counterfactuals}.
\end{itemize}

\todo{update for general soft}
%\subsection{Associated interventional data setting}


% \begin{figure}[h]
% \centering
% \begin{tikzpicture}

%   % Define nodes
%   \node[latent] (u) {$U^{(0)}$};
%   \node[latent, right= of u] (uc) {$U^{(c)}$};
%   \node[obs, below=of u]         (x) {$X^{(0)}$};
%   \node[latent, below=of uc]          (xc) {$\hat{X}^{(c)}$};
%   \node[obs, above=of uc] (c) {$C$};
%   \node[latent, above=of u]  (z) {$Z$};

%   % Connect the nodes
%   \edge {z} {u} ; %
%   \edge {z,c} {uc} ; %
%   \edge {u} {x} ; %
%    \edge {uc} {xc} ; %

%   % Plates
%   \plate {pa} {(c)(z)(x)} {$N$} ;
%   \plate {} {(pa)(c)(z)(x)} {$N_C$} ;

% \end{tikzpicture}
% \caption{Graphical model of the proposed causal?? VAE. Note that while $\hat{X}^{(c)}$ is not directly observed, we can compare it to marginal samples from $X^{(c)}$ via a discrepancy measure.  }
% \label{fig:VAE}
% \end{figure}

%\akash{See Figure 2 for alternative viz without the $N_C$ plate. I think Fig 1 is accurate but might be a little hard to read. Prob with Fig 2 is that it may give the wrong idea of the training, however, it does show that the training can be parallelized across contexts}




%Having established the latent variable causal model in Section \ref{sec:model}, now we present our VAE formulation for learning the model from data.


% In classical frequentist statistical modeling, the parameters $\theta$ of a model are estimated by maximizing the expectation of the model's loglikelihood under the data distribution, specifically
% \[
% \hat{\theta} = \arg\max_{\theta} \int p(x) \log p_\theta(x) dx,
% \]
% where $p_\theta(x)$ is the marginal likelihood of the model. 
% Unfortunately, in many instances obtaining the marginal $p_\theta(x)$ is not tractable, since we only have the conditional distribution $p_\theta(x | h)$.
% To remedy this issue, VAEs, introduced in \cite{kingma2013auto}, are designed to maximize the more tractable evidence lower bound (ELBO) under the data distribution, using amortized variational inference to train. The ELBO lower bounds the expected log likelihood as
% \begin{align}\nonumber
% &\int p(x) \log p_\theta(x) dx \geq \\&\mathbb{E}_{p(x)} \left[\mathbb{E}_{q_\phi(h|x)} [\log p_\theta(x|h)] - \mathrm{KL}(q_\phi(h|x) ||p(h))\right],\label{eq:elbo}
% \end{align}
% which only requires access to the conditional likelihood $p_\theta(x | h)$. The variational posterior $q_\phi(h|x)$ is been introduced with parameters $\phi$, and the second term of the ELBO encourages it to approach a desired distribution $p(h)$, which in our case is an isotropic Gaussian to encourage the elements of $h$ to be independent (disentangled).

%{\color{red} Kristjan: Remaining notation to establish here - $G$ needs to be upper triangular to enforce acyclicity, and we need $c$ to be encoded via a neural network. This is needed even if one assumes the node intervened is known - because the topological order is not known.}

%\subsection{Notation and Model Architecture}
We first describe how we incorporate the latent graphical model\footnote{Note that we refer to the relationship between $U,I$ and $X$ as the latent graphical model.} of Section \ref{sec:setup} into the VAE framework. 
%
For simplicity of illustration, we assume that the structural causal model (SCM) corresponding to the model in Eq.~\eqref{eq:modelnew} for $U$ is linear with additive noises, i.e. each $U_i$ is a linear function of its parents in $\mathcal{G}$ plus an exogenous noise term $Z_i$ (we do not need to assume the distribution of the $Z_i$ here). All the $Z_i$'s are mutually independent. 
%
The framework naturally extends to general non-linear SCMs with arbitrary noises which are presented in detail in Appendix \ref{append:consistent}.

% Due to the nonlinear encoding from the latent $U$ to the observed $X$ \eqref{eq:modelnew}, not much expressive power is lost. 
% \jq{add sentence about nonlinearity}

Our high-level approach is to encode observational samples $X^{\varnothing}$ into the independent exogenous factors $Z$ of the latent graphical model.
%
We then learn the parameters of the linear SCM to map these exogenous factors $Z$ to the (intervened) latent factors $U$, using the rules of interventional calculus. This structure allows us to generate counterfactual samples $X^{I}$ corresponding to individual observational samples $X^{\varnothing}$, for any desired intervention $I$. 



%PUT NON-ORDERED LINEAR SCM WITH INVERSE HERE FIRST?
Since the directed graph describing an SCM must be \emph{acyclic}, our architecture must enforce an acyclicity constraint. While optimization-based acyclicity constraints are available (e.g. \cite{zheng2018dags}), these add significant complexity to the optimization problem. Instead, we exploit the fact that we can only identify the latent nodes up to permutations (Definition~\ref{def:meq}), to assume without loss of generality that the latent factors $U_i$ are \emph{topologically ordered}, i.e., $i \to j$ implies $i < j$.
For $U_i$ topologically ordered, the linear SCM over $U$ can be characterized by an upper-triangular $G \in \mathbb{R}^{p \times p}$ where $G_{ij}$, is nonzero iff the DAG $\mathcal{G}$ contains an edge pointing from $i$ to $j$.
%
% Since the directed graph describing an SCM must be \emph{acyclic}, our framework must enforce an acyclicity constraint. While optimization-based acyclicity constraints are available (e.g. \cite{zheng2018dags}), these add significant complexity to the optimization problem. Instead, we exploit the fact that we do not know the identities of the latent nodes, to assume without loss of generality that the latent factors $U_i$ are \emph{topologically ordered}. 
% For $U_i$ topologically ordered, it can be shown that the linear SCM can be characterized as the set $(G, \{Z_i\}_{i=1}^p)$, where $G \in \mathbb{R}^{p \times p}$ is an upper triangular matrix\footnote{Specifically, $G_{ij} = 0$ for all $j > i$.}  where the element $G_{ij}$, $j > i$ is nonzero iff the DAG $\mathcal{G}$ contains an edge pointing from $V_i$ to $V_j$. 
%
Importantly, any matrix upper-triangular $G$ describes an acyclic graph. With this topological ordering, the overall model can be defined (recursively) as
\begin{equation}
    \begin{aligned}
        U_j\!\! &=\! (U_1, \!.., \!U_{j-1}) G_{1:j-1, j}\! +\! Z_j, \\
        \:X\! \!&=\! f(U_1, \!.., \!U_p)\label{eq:Model}
    \end{aligned}
\end{equation}

% Importantly, any matrix $G$ satisfying this upper triangular constraint describes an acyclic graph. With this topological ordering, we can define the $U_i$ recursively as
% \[
% U_j = [U_1, \dots, U_{j-1}] \cdot G_{:j-1, j} + Z_j.
% \]
% The overall model can then be summarized as
% \begin{align}
% \nonumber
% \mathrm{For \:} j &= 1,\dots, p \mathrm{:}\\ U_j &= [U_1, \dots, U_{j-1}] G_{:j-1, j} + Z_j,\quad X = f(U_1, \dots, U_p).\label{eq:Model}
% \end{align}
%To recap, the number of latent variables is $p$, the latent variables are the $U_i$, the exogenous noise variables are the $Z_i$, $G$ is an upper triangular matrix encoding the linear SCM, and $f(\cdot)$ is a deterministic, possibly nonlinear transformation mapping the causally related latent variables $U$ to the observed vector $X$.

\begin{wrapfigure}{r}{0.17\textwidth} 
\centering
\resizebox{\linewidth}{!}{
\begin{tikzpicture}

  % Define nodes
  \node[latent, minimum size=1cm] (u) {$U^\varnothing$};
  \node[latent, right= of u, minimum size=1cm] (uc) {$U^{\{1\}}$};
  \node[latent, right= of uc, minimum size=1cm] (uc1) {$U^{\{K\}}$};
  
  
  \node[obs, below=of u, minimum size=1cm] (x) {$X^{\varnothing}$};
  \node[obs, below=of uc, minimum size=1cm] (xc) {${X}^{\{1\}}$};
  \node[obs, below=of uc1, minimum size=1cm](xc1) {${X}^{\{K\}}$};
  \node at ($(uc)!.5!(uc1)$) {\ldots};
  
  \node[obs, above=of uc, minimum size=1cm] (c) {$C^{\{1\}}$};
  \node[obs, above=of uc1, minimum size=1cm] (c1) {$C^{\{K\}}$};
  \node[latent, above=of u, minimum size=1cm]  (z) {$Z$};

  % Connect the nodes
  \edge {z} {u} ; %
  \edge {z,c} {uc} ; %
  \edge {z,c1} {uc1} ; %
  \edge {u} {x} ; %
   \edge {uc} {xc} ; %
   \edge {uc1} {xc1} ; %

  % Plates
  %\plate {pa} {(c)(z)(x)(xc1)} {$N$} ;
  % \plate {} {(pa)(c)(z)(x)} {$N_C$} ;

\end{tikzpicture}
}
\caption{Graphical representation of our proposed model, where $K$ separate interventions $C^{\{k\}}$ are indicated.  }
%Note that we only have training samples from the marginal distributions of $X^{(0)}, X^{(c_k)}$ instead of the joint distribution. Hence our model infers the latent exogenous factor $Z$ from observational samples $X^{(0)}$, and generates corresponding interventional samples for each of the desired interventions $C^{(k)}$.
\vspace{-.1in}
\label{fig:VAE}
\end{wrapfigure}


\textbf{Interventions.} 
%A variety of possible intervention types exist, including \emph{hard} interventions that fix a node to a chosen value and eliminate the impact of its parents, or \emph{soft} interventions that perturb the causal mechanism that creates the node. 
In this discussion, we focus on \emph{shift} interventions.
%
The extension to hard interventions is straightforward and can be found in Appendix \ref{append:consistent}. 
A single-node shift intervention in our model \eqref{eq:Model} adds $a_i$ to the equation for node $i$, $U_i = [U_1,\dots,U_{i-1}] G_{1:i-1,i} + Z_i + a_i$, and keeps the remaining node mechanisms unchanged.

Generalizing this to interventions at multiple nodes, with a slight abuse of notation, let $I = \{ (i, a_i) \}_{i\in I}$ denote the set of active interventions, where node(s) $i\in I$ are perturbed by shift(s) $a_i$. We can then replace \eqref{eq:Model} with
% \begin{align} \nonumber
% U^{(C)}_i &= \left\{\begin{array}{ll} \left[U^{(C)}_1, \dots, U^{(C)}_{i-1}\right] G_{:i-1, i} + Z_i + \delta_i, & i \in \{V_j\} \\  
% \left[U^{(C)}_1, \dots, U^{(C)}_{i-1}\right] G_{:i-1, i} + Z_i, & i \notin \{V_j\}\end{array}\right.\\
% % U_{i} &= \mu_i\\
% % \mathrm{For } &j \notin c \mathrm{:}\: U_j = [U_1, \dots, U_{j-1}] G_{:j-1, j} + Z_j,\quad 
% X^{(C)} &= f(U_1, \dots, U_L),
% \label{eq:ModelInt}
% \end{align}
\begin{align} \nonumber
U^{I}_j &= \left[U^{I}_1, \dots, U^{I}_{j-1}\right] G_{1:j-1, j} + Z_j + a_j\kron_{j \in I},
\\
% U_{i} &= \mu_i\\
% \mathrm{For } &j \notin c \mathrm{:}\: U_j = [U_1, \dots, U_{j-1}] G_{:j-1, j} + Z_j,\quad 
X^{I} &= f(U_1^I, \dots, U_p^I).
\label{eq:ModelInt}
\end{align}
%generating the $U_i$ and $X$ iteratively as before.

% In our model \eqref{eq:Model}, a \emph{soft shift intervention} perturbing node(s) $V_j$ by shift(s) $\mu_j$ corresponds to replacing the structural equation $U_{V_j} = [U_1, \dots, U_{V_j-1}] G_{:V_j-1, V_j} + Z_{V_j}$ in \eqref{eq:Model} with $U_{V_j} = \mu_j$, i.e.


Given an intervention $I=\{ (i, a_i) \}_{i\in I}$, it is convenient to define the shift vector $\mathbf{a}_I = [a^{I}_1,\dots, a^{I}_p]$ such that 
\[
a^{I}_i = \left\{\begin{array}{ll} a_i, & i \in I \\  
0, & i \notin I.\end{array}\right.
\]
Hence the elements of the shift vector $\mathbf{a}_I$ describe the amount each of the $p$ nodes is shifted. 
Adopting the convention $\mathbf{a}_\varnothing = 0$ (i.e. the observational case $I = \varnothing$ with no perturbations), we can then unify the observational case \eqref{eq:Model} and the intervened case \eqref{eq:ModelInt} in a single matrix equation $U^{I} = U^{I} G + Z + \mathbf{a}_I$,
which yields 
\begin{equation}
\label{eq:Gs}
U^{I} = (Z + \mathbf{a}_I) (\mathbf{I}_p - G)^{-1},
\end{equation}
where $\mathbf{I}_p\in\bbR^{p\times p}$ is the identity matrix and recall the observational case is denoted by $U^{\varnothing}$, $X^{\varnothing}$.
% intervention-modified graph adjacency matrix $G^{(c)} \in \mathbb{R}^{(c)}$
% \[
% G^{(c)}_{:, i} = \left\{\begin{array}{ll} G_{:i} & i \notin c \\ 0 & i \in c\end{array}\right.
% \]
% and 
% exogenous vector $Z^{(c)} \in \mathbb{R}^p$ such that
% \[
% Z^{(c)}_i = \left\{\begin{array}{ll} Z_i & i \notin c \\ \mu_c & i \in c\end{array}\right.,
% \]
% yielding for any $c$ (since $G^{(c)}$ is upper triangular)
% \[
% U = U G^{(c)} + Z^{(c)}
% \]
% implying
% \begin{equation}
% \label{eq:Gs}

% U = Z^{(c)} (I - G^{(c)})
% \end{equation}
% where we use the convection $G^{(0)} = G$ and $Z^{(0)} = Z$.

%\paragraph{Encoding interventions}
% In the above, for simplicity of presentation the interventions $C$ were given. In practice, it is nearly always the case that it is not known which latent variable was intervened on. In such settings, we assume that the number of intervened nodes $m$ is given, and separate metadata $I_j$ describing each of the $j=1,\dots,m$ active interventions is available. 
Recalling that we are not directly given the interventions $I$ in practice and are instead given some additional label $C$ (e.g., the superscript of $\cD^1$ in Section \ref{sec:setup}), we must learn a map from $C$ to $I$:
\begin{equation}
\label{eq:intervEnc}
I = \phi(C).
\end{equation}
Here, $\phi$ is shared across different distributions. For single-node intervention $I = \{(j, a_j)\}$, we encode $j$ as a one-hot vector and $a_j$ as a scalar. This formulation allows us to easily encode multi-node interventions, by encoding each node's intervention using \eqref{eq:intervEnc} and concatenating the results. For simplicity, we will denote $I$ instead of another notation as the encoded $\phi(C)$. The places where $I$ refers to $\phi(C)$ instead of the ground-truth intervention $I$ should be evident. Figure \ref{fig:VAE} summarizes the latent graphical model.

\textbf{Likelihood and the ELBO.}
%To obtain the ELBO for our approach, we first establish notation for the necessary likelihoods under our generative model in Section \ref{sec:model}. 
We have data distributions $\bbP(X^{I})$, where recall $I$ is a variable indicating the intervention of choice. We let $\bbP(I)$ be a distribution established on $I$ (typically uniform over discrete sets of $I \neq \varnothing$ available in the dataset). We assume we have $N$ samples $\{X_i^{\varnothing}\}_{i=1}^N$ from the observational distribution $X^{\varnothing}$, and for each intervention $I$, we assume we have $N_I$ samples $\{X^{\varnothing}_i\}_{i=1}^{N_I}$ from $X^{I}$.
%\footnote{These are equal for simplicity of notation, unequal numbers of samples are allowed.} 

We let $\hat{Z}$ be the learned latent exogenous factors $Z$ sampled from an encoder $q_{\phi}(\hat{Z}|X^{\varnothing})$, as our goal is to have these factors be independent (disentangled). Recall the shift vector $\mathbf{a}_I$. By \eqref{eq:Gs}, our decoder likelihood can then be written in the form
\begin{align}
p_{\theta,\varnothing}(X^{\varnothing} | \hat{Z}) &= p_\theta(X^{\varnothing} | \hat{U} = \hat{Z} (\mathbf{I}_p - G)^{-1})\nonumber\\
p_{\theta, I} (X^{I} | \hat{Z}) &= p_\theta(X^{I} | \hat{U}^{I} = (\hat{Z} + \mathbf{a}_I) (\mathbf{I}_p - G)^{-1}).\label{eq:uh}
\end{align}
%ESTABLISH THIS INVERSE STUFF EARLIER
% where $\bbP_\theta(X | U)$ is shared for all $I$.

Following the architecture shown in Figure \ref{fig:modelUn}, for observational input $X^{\varnothing}$, once $\hat{Z}$ is obtained, our model reconstructs the input (via $p_{\theta,\varnothing}(X^{\varnothing} | \hat{Z})$), as well as produces counterfactual samples for each $I$ (via $p_{\theta, I} (X^{I} | \hat{Z})$). 

\paragraph{Paired data setting} For the simpler setting where for each sample from $X^{\varnothing}$ there exist corresponding samples for $X^{I}$, the ELBO can then be immediately written as
\begin{align}
\nonumber
&\mathbb{E}_{\bbP(I)} \log \bbP(X^{\varnothing}, X^{I}) \geq \\\label{eq:ELBOassoc}&\mathbb{E}_{\bbP(I)}\left\{\mathbb{E}_{\bbP(X^{\varnothing}, X^{I})} \Big[\mathbb{E}_{q_\phi(\hat{Z}|X^{\varnothing})} \log p_{\theta,\varnothing}(X^{\varnothing}|\hat{Z})+\right. \\&\left. \mathbb{E}_{q_\phi(\hat{Z}|X^{\varnothing})} \log p_{\theta,I}(X^{I}|\hat{Z}) - D_{KL}\big(q_\phi(\hat{Z}|X^{\varnothing}) ||p(\hat{Z})\big)\Big]\right\},\nonumber
\end{align}
% \begin{equation}
%     \begin{aligned}
%     &\mathbb{E}_{p(c)} \log p(x^{(0)}, x^{(c)}) \geq \\\nonumber&\mathbb{E}_{p(c)}\left[\mathbb{E}_{p(x^{(0)}, x^{(c)})} \left[\mathbb{E}_{q_\phi(h|x^{(0)})} [\log p_{\theta,0}(x^{(0)}|h)]\right.\right. \\&\left.\left.+ \mathbb{E}_{q_\phi(h|x^{(0)})} [\log p_{\theta,c}(x^{(c)}|h)] - \mathrm{KL}(q_\phi(h|x^{(0)}) ||p(h))\right]\right],\label{eq:ELBOassoc}
%     \end{aligned}
% \end{equation}

where we have used the fact that $X^{\varnothing}$ and $X^{I}$ are independent given $\hat{Z}$. Here $p(\hat{Z})$ is a factored prior chosen for independent exogenous noises.

\begin{figure}
    \centering
    \vspace{-.1in}
    \includegraphics[width=.95\linewidth]{fig/shiftcausalvae_architecture.pdf}
%     \begin{tikzpicture}[
% roundnode/.style={circle, draw=black!60,  very thick, minimum size=7mm},
% squarednode/.style={rectangle, draw=black!60,  very thick, minimum size=5mm},
% ]
% %Nodes
% \node[squarednode]        (start)        {Input $X^{(0)}$};
% \node[squarednode]        (c)    [right=of start]    {Intervention $c$};
% \node[squarednode]        (z)       [below=of start] {Exogenous $Z$};
% \node[squarednode]        (vc)       [below=of c] {Encoded interv. $(v, \delta)$};
% \node[squarednode]        (data)   [right=of vc]     {Interv. Data $X^{(c)}$};
% \node[squarednode]        (u)       [below=of z] {Latent recon. $U^{(0)}$};
% \node[squarednode]        (uc)       [below=of vc] {Interv. latent $U^{(c)}$};
% \node[squarednode]        (recon)       [below=of u] {Recon. $\hat{X}^{(0)}$};
% \node[squarednode]        (interv)       [below=of uc] {Interv. $\hat{X}^{(c)}$};
% \node[squarednode]        (lossrecon)       [left=of recon] {L2 recon loss};
% \node[squarednode]        (lossMMD)       [right=of interv] {MMD loss};
% %Lines
% \draw[->] (start.south) -- (z.north);
% \draw[->] (c.south) -- (vc.north);
% \draw[->] (z.south) -- (u.north);
% \draw[->] (z.south) -- (uc.north);
% \draw[->] (c.south) -- (data.north);
% \draw[->] (vc.south) -- (uc.north);
% \draw[->] (u.south) -- (recon.north);
% \draw[->] (uc.south) -- (interv.north);
% \draw[->] (recon.west) -- (lossrecon.east);
% \draw[->] (start.south) -- (lossrecon.north);
% \draw[->] (interv.east) -- (lossMMD.west);
% \draw[->] (data.south) -- (lossMMD.north);
% %\draw[->] (maintopic.east) -- (rightsquare.west);
% %\draw[->] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (lowercircle.east);
% \end{tikzpicture}
    \caption{\textbf{Discrepancy VAE architecture.} Input samples $X^{\varnothing}$ are encoded into exogenous variables $Z$, which are transformed via causal graph into the latent variables $U^{\varnothing}$ and the intervened $U^{I}$. Then, $U^{\varnothing}$ and $U^{I}$ are decoded into $\hat{X}^{\varnothing}$ and $\hat{X}^{I}$, respectively. $l_2$ reconstruction loss and MMD loss are used to compare to the corresponding datasets.  }
    \label{fig:modelUn}
    \vspace{-.2in}
\end{figure}

\paragraph{Unpaired data setting} 
%The main focus of this work, however, is on the unpaired setting where the observational data $X^{\varnothing}$ and the interventional data $X^{I}$ do not have correspondence. 
In the unpaired setting, however, we do not have samples from $\bbP(X^{\varnothing}, X^{I})$ and hence cannot compute the expectation in the second term of \eqref{eq:ELBOassoc}. More intuitively, we cannot directly compare individual samples of $X^{I}$ to the samples $\hat{X}^{I}$ that our model generates from $X^{\varnothing}$. Instead, we can only compare their distributions. We, therefore, propose to replace the second term in \eqref{eq:ELBOassoc} with a discrepancy measure between the \emph{distributions}, specifically,
\begin{align}
\nonumber
&\mathbb{E}_{\bbP(I)}\left\{\mathbb{E}_{\bbP(X^{\varnothing})} \Big[\mathbb{E}_{q_\phi(\hat{Z}|X^{\varnothing})} \log p_{\theta,\varnothing}(X^{\varnothing}|\hat{Z}) \right. \\&\left.- D_{KL}\big(q_\phi(\hat{Z}|X^{\varnothing}) ||p(\hat{Z})\big)- \alpha D\big(\{\hat{X}^{I}\} , \{X^{I}\}\big)\Big]\right\},\label{eq:ELBOunassoc}
\end{align}
where $D(\cdot, \cdot)$ is a chosen discrepancy measure (computed on samples of $\hat{X}^{I} , X^{I}$), and $\alpha$ is a weighting parameter. 


There are a wide variety of possible discrepancy measures that can be used here. To avoid the saddle point optimization challenges that come with adversarial training, we do not consider adversarial methods such as those utilized in GANs (e.g. the dual form of the Wasserstein distance in \cite{arjovsky2017wasserstein}). This leaves non-adversarial discrepancy measures that (for optimization to proceed) must be computationally efficient, differentiable, and possible to optimize via common variants of stochastic gradient descent. Popular discrepancy measures that fit these criteria include the MMD (Maximum Mean Discrepancy) \cite{gretton2012kernel}, the entropic Wasserstein distance \cite{frogner2019learning}, and the Sliced Wasserstein distance \cite{wu2019sliced}. In this work, we focus on the MMD. 

For $D(\cdot,\cdot)$ being the MMD with Gaussian kernel of width $\epsilon$ sufficiently large, we can show that Eq.~\eqref{eq:ELBOunassoc} with an appropriate choice of $\alpha$ in fact is a lower bound to Eq.~\eqref{eq:ELBOassoc}, and is therefore also a lower bound to the off-the-shelf paired log-likelihood. We state an informal version of this here, where the full version and the proof of the following are in Appendix \ref{app:elbo}.  \looseness=-1 

\begin{proposition}[Likelihood Lower Bound, Informal]\label{thm:elbo}
Up to an additive constant, Eq.~\eqref{eq:ELBOunassoc} lower bounds the paired-data ELBO in Eq.~\eqref{eq:ELBOassoc} and by extension the paired-data log-likelihood $\mathbb{E}_{\bbP(I)} \log \bbP(X^{\varnothing}, X^{I})$.
\end{proposition}







% Specifically, in this work we seek to maximize the following loss:
% \begin{align}
% \nonumber
%  &\mathbb{E}_{p(c)}\left[\mathbb{E}_{p(x^{(0)})} \left[\mathbb{E}_{q_\phi(h|x^{(0)})} [\log p_{\theta,0}(x^{(0)}|h)]  \right.\right. \\&\left.\left.- \beta\mathrm{KL}(q_\phi(h|x^{(0)}) ||p(h))\right]+ \alpha D\left(\hat{X}^{(c)} , X^{(c)}\right)\right],\label{eq:ELBOunassocBeta}
% \end{align}
% where the weights $\alpha$, $\beta$ are hyperparameters.



%While the main focus of this work is on the unassociated setting where the observational data $X^{(0)}$ and the interventional data $X^{(c)}$ do not have correspondence, to aid intuition we first introduce the model for the simpler associated setting where each interventional data point in $X^{(c)}$ has a corresponding unintervened $X^{(0)}$ sample that shares exogenous variables.






% \begin{figure*}
%     \centering
%     \begin{tikzpicture}[
% roundnode/.style={circle, draw=black!60,  very thick, minimum size=7mm},
% squarednode/.style={rectangle, draw=black!60,  very thick, minimum size=5mm},
% ]
% %Nodes
% \node[squarednode]        (start)        {Input $X^{(0)}$};
% \node[squarednode]        (c)    [right=of start]    {Intervention $c$};
% \node[squarednode]        (z)       [below=of start] {Exogenous $z$};
% \node[squarednode]        (vc)       [below=of c] {Encoded hard interv. $v_c$};
% \node[squarednode]        (data)   [right=of vc]     {Interv. Data $X^{(c)}$};
% \node[squarednode]        (u)       [below=of z] {Latent recon. $u$};
% \node[squarednode]        (uc)       [below=of vc] {Interv. latent $u_c$};
% \node[squarednode]        (recon)       [below=of u] {Recon. $\hat{X}^{(0)}$};
% \node[squarednode]        (interv)       [below=of uc] {Interv. $\hat{X}^{(c)}$};
% \node[squarednode]        (lossrecon)       [left=of recon] {L2 recon loss};
% \node[squarednode]        (lossMMD)       [right=of interv] {L2 recon loss};
% %Lines
% \draw[->] (start.south) -- (z.north);
% \draw[->] (start.south) -- (data.north);
% \draw[->] (c.south) -- (vc.north);
% \draw[->] (z.south) -- (u.north);
% \draw[->] (z.south) -- (uc.north);
% \draw[->] (c.south) -- (data.north);
% \draw[->] (vc.south) -- (uc.north);
% \draw[->] (u.south) -- (recon.north);
% \draw[->] (uc.south) -- (interv.north);
% \draw[->] (recon.west) -- (lossrecon.east);
% \draw[->] (start.south) -- (lossrecon.north);
% \draw[->] (interv.east) -- (lossMMD.west);
% \draw[->] (data.south) -- (lossMMD.north);
% %\draw[->] (maintopic.east) -- (rightsquare.west);
% %\draw[->] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (lowercircle.east);
% \end{tikzpicture}
%     \caption{Model for associated intervention data - TO DO LABEL EDGES AND MAKE NICER }
%     \label{fig:modelMSE}
% \end{figure*}

% \subsection{Unassociated interventional data setting}
% Having presented the framework in the simpler associated setting, we now turn to the unassociated setting which is the main focus of this work. 

% The Causal VAE framework in this setting is summmarized in Figure \ref{fig:modelUn}. Note that since the interventional data $X^{(c)}$ is no longer associated with corresponding $X^{(0)}$ samples, there is no longer an edge connecting them in Figure \ref{fig:modelUn}. 

% As a result, the reconstruction loss cannot be used between the estimated intervention $\hat{X}^{(c)}$ (which derives from $X^{(0)}$) and the interventional data $X^{(c)}$ since they do not share exogenous variables. Instead, we must use a \emph{distributional loss}, which measures the difference between the corresponding \emph{distributions}. Specifically,
% \[
% distributional loss.
% \]




%DESCRIBE VAE LOSS ETC

% \begin{theorem}[Consistency of the loss function]
% Assume universal approximation and ..., the unique minimizer of loss function x acheives $\cA$-idenfiability.
% \end{theorem}


The full discrepancy-based VAE framework is summarized in Figure \ref{fig:modelUn}.
%
In fact, this framework is also \emph{consistent}, i.e., it recovers the $\cM$-equivalence class proven in Corollary~\ref{cor:1} and Theorem~\ref{thm:1} in the infinite sample regime. We show formal proofs in Appendix~\ref{append:consistent}.

==> content/old/experiments-old.tex <==
\section{Experiments}
\label{sec:experiments}

\todo{clean up}
%\subsection{Discrepancy VAE Implementation}



%Code for our method is at \url{https://anonymous.4open.science/r/causaldiscrepancyvae-72AC}.

\subsection{Synthetic Data}\label{sec:experiments1}

Consider a synthetic dataset in 50-dimensional space, where $p$ latent factors generated by a linear causal chain graph with additive Gaussian noises are embedded in 50-dimensional space via a random linear map. For training, we generate 5000 unpaired samples from the distributions of the observational $X^{\varnothing}$ and each of the intervened $X^{I}$, where we consider $p$ single-node interventions, one for each of the $p$ latent factors. 


For testing, we generate 1000 paired $(X^{\varnothing}, X^{I})$ samples for a set of unseen interventions including (a) every single-node intervention and (b) every double-node intervention. %The intervention sizes at test time are different than at train time. 
The paired training data allows us to evaluate whether the model has successfully learned to generate paired samples. We evaluate the model with 4 metrics: (1) the recovery of the true causal graph as measured by probabilities of detection and false alarm, (2) the normalized RMSE of reconstructing the observational test samples, (3) the normalized RMSE of predicting the paired test samples of single-node interventions, and (4) the normalized RMSE of predicting the paired test samples of double-node interventions. The probabilities of detection (PD) and false alarm (PFA) for graph recovery are computed based on individual edges in the graph.\footnote{Note that a random strategy of choosing edges at random with probability $\epsilon$ yields a PD and PFA both equal to $\epsilon$.}

The implementation details and code are provided in Appendix \ref{app:implementation}. We summarize the results for both hard interventions and shift interventions in Table \ref{fig:synth}. We repeated the experiment in Table \ref{fig:synthNonlin} with a nonlinear decoder\todo{i don't understand the reason for using a more expressive decoder? KG Answer: this demonstrates the model does not need to know that the true model is linear in order to succeed. In other words, a robustness test.} (the true model remained linear), with the decoder also being 2-layer with 128 hidden units. Throughout, we used weight $\alpha = 1$ in \eqref{eq:ELBOunassoc}. Both experiments achieved low RMSE on the single-node interventional data, despite only training on unpaired samples. Generalization to double-node interventions is successful in both settings despite only seeing single-node interventions in training. The edge recovery probabilities are significantly better than random especially for smaller $p$. 
%
For the RMSE metrics, having a more complex decoder (or even having larger $p$) does not seem to consistently degrade performance.
%
However, the graph estimation degrades for larger $p$ when using a more expressive decoder.
% \begin{table*}
% \centering
% \footnotesize
%For graph edge detection there is a degradation in performance as $p$ increases, and it seems that in general having a nonlinear decoder when the true embedding is linear is moderately disadvantageous, as might be expected. 

% \label{fig:synthNonlin}
% \end{table*}



% linear-linear model with shift interventions and random graph (edges prop to nodes). X axis - 4 different values of p, e.g. 5, 10, 15, 20. Three lines: recon error, avg 1-node interv error, avg 2-node interv error. 

% Second figure: hard interventions

% \paragraph{Hard interventions} The results for hard interventions are sh

% \paragraph{Shift interventions}

\begin{table}[h]
\centering
\begin{subtable}[t]{\linewidth}
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{ p{1.5cm}|p{1.5cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}||p{1.5cm}|p{1.5cm} } 
 \hline
 \textbf{Intervention Type} & \textbf{\# of latents} & \textbf{Baseline RMSE ($\downarrow$)} & \textbf{1-node RMSE ($\downarrow$)} & \textbf{2-node RMSE ($\downarrow$)} & \textbf{Edge PD ($\uparrow$)} & \textbf{Edge PFA ($\downarrow$)} \\ 
 \hline\hline
 \textbf{Shift} & {${p=5}$} & 0.47 & 0.47 & 0.70 & 0.75 & 0 \\ 
 \hline
   & {${p=10}$} & 0.37 & 0.33 & 0.46 & 0.9 & 0.16 \\ 
 \hline
   & {${p=15}$} & 0.27 & 0.33 & 0.43 &  0.71 & 0.39 \\ 
 \hline\hline
  \textbf{Hard} & {${p=5}$} & 0.21 & 0.36 & 0.71 & 0.75 & 0 \\ 
 \hline
   & {${p=10}$} & 0.14 & 0.35 & 0.53 & 0.78 & 0.33 \\ 
 \hline
   & {${p=15}$} & 0.28 & 0.51 & 0.67 &  0.79 & 0.45  \\ 
 \hline
\end{tabular}}
\caption{Linear-linear: The VAE decoder is set to be linear, matching the ground truth.   }
\label{fig:synth}
\end{subtable}
\hspace{\fill}
\begin{subtable}[t]{\linewidth}
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{ p{1.5cm}|p{1.5cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}||p{1.5cm}|p{1.5cm}} 
 \hline
 \textbf{Intervention Type} & \textbf{\# of latents} & \textbf{Baseline RMSE ($\downarrow$)} & \textbf{1-node RMSE ($\downarrow$)} & \textbf{2-node RMSE ($\downarrow$)} & \textbf{Edge PD ($\uparrow$)} & \textbf{Edge PFA ($\downarrow$)} \\ 
 \hline\hline
 \textbf{Shift} & {${p=5}$} & 0.40 & 0.30 & 0.68 & 0.75 & 0.17 \\ 
 \hline
   & {${p=10}$} & 0.36 & 0.36 & 0.51 & 0.78 & 0.44  \\ 
 \hline
   & {${p=15}$} & 0.29 & 0.57 & 0.68 & 0.79 & 0.42 \\ 
 \hline\hline
  \textbf{Hard} & {${p=5}$} & 0.44 & 0.39 & 0.59 & 0.75 & 0.17 \\ 
 \hline
   & {${p=10}$} & 0.32 & 0.50 & 0.70 & 0.78 & 0.25 \\ 
 \hline
   & {${p=15}$} & 0.29 & 0.53 & 0.70 & 0.57 & 0.44  \\ 
 \hline
\end{tabular}}
\caption{Linear-nonlinear: The VAE decoder is set to be a \textbf{nonlinear} neural network, i.e. more expressive than the ground truth. }
\label{fig:synthNonlin}
\end{subtable}
\caption{Performance on a synthetic dataset with $p$ latent variables and linear embedding into 50 dimensional space. 
% Generalization to 2-node interventions is successful in both settings despite only seeing 1-node interventions in training, and the edge recovery probabilities are significantly better than random especially for smaller $p$. The more expressive nonlinear decoder has the downside, however, that graph estimation degrades for larger $p$.
}
% \vspace{-.2in}
%\label{fig:synth}
\end{table}


\subsection{Biological Data}\label{sec:experiments2}
We next apply our method to real-world biological data. For this, we use the large-scale Perturb-seq study from \cite{norman2019exploring}. After pre-processing, it contains 8907 unperturbed cells (observational distribution $\cD$) and 99590 perturbed cells that underwent CRISPR activation \cite{gilbert2014genome} targeting one or two out of 105 genes (interventional distributions $\cD^1$,...,$\cD^K$). CRISPR activation experiments modulate the expression of its target genes, which we model as a shift intervention. Each interventional distribution comprises 50 to 2000 cells. Each cell is represented as a 5000-dimensional vector (observed variable $X$) measuring the expressions of 5000 highly variable genes. 

To test our model, we set the latent dimension $p=105$, which corresponds to the total number of targeted genes. During training, we include all the unperturbed cells from the observational distribution $\cD$ and the perturbed cells from the single-node interventional distributions $\cD^1,...,\cD^{105}$ that target one gene. We randomly extract 96 cells from all single-node interventional distributions with more than 800 cells and reserve these for testing. The double-node interventions (112 distributions $\cD^{106},...,\cD^{218}$) targeting two genes are entirely reserved for testing. The following results summarize the model with the best training performance.\footnote{The training performance is determined by Eq.~\eqref{eq:ELBOunassoc} with $\alpha=1$.} Extended evaluations and detailed implementation can be found in Appendix \ref{append:c}.


\textbf{Single-node Interventional Distributions.} To study the generated samples of the VAE for interventions targeting a single gene, we generate $96$ samples for each single-node intervention that has more than 800 cells (14 distributions). 
%
These are compared against the left-out $96$ cells of the corresponding distributions. 
%
Figure \ref{fig:7} illustrates this for $3$ example genes in 2 dimensions using UMAP~\cite{mcinnes2018umap} with all other cells in the dataset as background (labeled by ‘NA’). 
%
Interestingly, our model is able to discover subpopulations of the interventional distributions (e.g., for `KLF1', the generated samples are concentrated in the middle left corner). 
%
We provide a quantitive evaluation for all $105$ single-node interventions in Figure \ref{fig:8}. 
%
The model is able to obtain close to perfect $R^2$ (on average 0.99 over all genes and 0.95 over most differentially expressed genes) for all perturbations on single genes. %\textcolor{red}{How well do you do on unseen single gene interventions?}

\begin{figure*}[tb]
    \centering
    \vspace{-.1in}
\includegraphics[width=.85\textwidth]{fig/fig-sample_single_example.pdf}
% \vspace{-.2in}
    \caption{UMAP visualization of the generated samples vs. the ground-truth samples. Left: all 14 single target-node interventions with more than $800$ cells. Middle-Right: distributions for target genes `SET', `CEBPE', and `KLF1'.}
    \label{fig:7}
\end{figure*}

\begin{figure}[h]
    \centering
\includegraphics[width=.42\textwidth]{fig/fig-rm_single.pdf}
\vspace{-.1in}
    \caption{RMSE and $R^2$ of all $105$ single target-gene interventions. `all genes' indicates measurements using the entire $5000$-dimensional vectors; `DE genes' indicates measurements using the $20$-dimensional vectors on top $20$ most differentially expressed genes.}
    \label{fig:8}\vspace{-.2in}
\end{figure}


\textbf{Double-node Interventional Distributions.} Next, we analyze the generalization capabilities of our model to the $112$ double-node interventions. Despite never observing any cells from these interventions during training, we obtain reasonable $R^2$ values (on average 0.94 over all
genes and 0.70 over most differentially expressed genes).
% as compared to the reported results in previous works (e.g.~Supplementary Fig.~2 in \cite{lotfollahi2021learning}) that trained an adversarial model using all but $13$ double gene interventions \textcolor{red}{What did they obtain?}.
However, when looking at the generated samples for individual pairs of interventions, it is apparent that our model performs well on some pairs, but recovers different subpopulations for others (examples shown in Figure \ref{fig:9} in Appendix \ref{append:c}). The wrongly predicted intervention pairs could indicate that the two target genes act non-linearly, which needs to be further evaluated and is of independent interest for biological research \cite{horlbeck2018mapping,norman2019exploring}.


\textbf{Structure Learning.} Lastly, we examine the learned DAG between the intervention targets. Specifically, this corresponds to a learned gene regulatory network between the learned programs of target genes. For this, we reduce $p$ from $105$ until the learned latent targets of $\cD^1,...,\cD^{105}$ using Eq.~\eqref{eq:intervEnc} cover all $p$ latent nodes. This results in $p=7$ groups of genes, where genes are grouped by their learned latent nodes. The learned DAG over these groups is demonstrated with example genes in Figure \ref{fig:6} (left).
% We focus on 6 out of the 105 target genes whose interventional distributions have more than $800$ cells  and distribution means that are significantly different than the observational distribution.\footnote{This is measured by the $l_1$-distance between two mean vectors.} The rationale behind this second condition is to avoid noise caused by non-effective knockdowns, which may result in erroneous directions \cite{zhang2022active}. 
% We also include $2$ genes `MAPK1' and `DUSP9', marked as important in \cite{norman2019exploring}. 
This learned structure is in accordance with previous findings. For example, we successfully identified the edges `DUSP9'$\rightarrow$'MAPK1' and `DUSP9'$\rightarrow$'ETS2', which is validated in \cite{norman2019exploring} (see their Fig.~5).
%
We also show the interventional distributions targeting these example genes in Figure \ref{fig:6} (right).
%
Among these, `MAPK1' and `ETS2' correspond to clusters that are heavily overlapped, which explains why the model maps both distributions to the same latent node. 


\begin{figure}[b]
    \centering
\includegraphics[width=.49\textwidth]{fig/fig-structure_learn.pdf}
% \vspace{-.2in}
    \caption{\textbf{Structure learning on the biological dataset.} Left: learned DAG between target genes (colors indicate edge weights). Right: UMAP visualization of the distributions.}
    \label{fig:6}
    \vspace{-.2in}
\end{figure}

==> content/old/identifiability.tex <==
\subsection{Hard Interventions}

Following \cite{ahuja2022interventional}, we can easily deduce $\cM$-identifiability given one hard intervention on each latent node, stated in the following corollary.

\begin{corollary}[Hard Intervention]\label{cor:1}
 Suppose Assumption \ref{assumption:1} holds true and observational data $\cD$ and interventional data $\cD^1,...,\cD^K$ from at least one hard intervention on each latent node are available, where each intervention targets one node and preserves support with the non-empty interior on all variables aside from its intervention target. The latent causal variables $U$, DAG $\cG$, and the intervention targets $I_1,...,I_K$ are identifiable up to their $\cM$-equivalence class.
\end{corollary}

The intuition of this corollary relies on the fact that the hard intervention corresponding to $\cD^i$ removes all incoming edges to its intervention target and sets it to one fixed value. Consider the simpler case where $K=p$: since $\cD^1,...,\cD^p$ corresponds to one hard intervention on each latent node, we should observe each of the latent variables taking a fixed value in one of $\cD^1,...,\cD^p$. By enforcing this constraint, we can recover both $U$ and $I_1,...,I_p$ up to equivalence classes. Together with $\cD,\cD^1,...,\cD^p$, this then recovers $\cG$ up to equivalence classes. 
%In general for $K\geq p$, several of $\cD^1,...,\cD^K$ would 

\subsection{Shift Interventions}

When considering shift interventions, the above arguments will not apply, since a shift intervention does not set its intervention target to a fixed value. In fact, it is not even possible to identify the latent variables $U$ up to its $\cM$-equivalence class: 

\begin{example}\label{exp:1}
Consider a $2$-node DAG $1\rightarrow 2$ as the true causal structure $\cG$. Assume the probability distribution of $U_1$ is $\cN(0,1)$ and the conditional probability distribution of $U_2$ given $U_1$ is $\cN(U_1,1)$. Further suppose that $f$ is the identity map, and that $\cD^1$ targets node $1$ with $\bbP^{\{1\}}_{U}(U_1)$ being $\cN(1,1)$, and $\cD^2$ targets node $2$ with $\bbP^{\{1\}}_{U}(U_2)$ being $\cN(U_1+1,1)$. Now consider a new set of latent variables \[\hat{U}=(U_1,U_1+U_2)\]
and a new function $\hat{f}(\hat{U})=(\hat{U}_1, \hat{U}_2 - \hat{U}_1)$ such that $\hat{f}(\hat{U})=U=f(U)=X$. The joint distribution in $\cD$ has factorization $\bbP(\hat{U}_1, \hat{U}_2)=\bbP(\hat{U}_1)\bbP(\hat{U}_2|\hat{U}_1)$ with $\bbP(\hat{U}_1)$ being $\cN(0,1)$ and $\bbP(\hat{U}_2|\hat{U}_1)$ being $\cN(2\hat{U}_1,1)$. $\cD^1$ only modifies $\bbP(\hat{U}_1)$ into $\cN(1,1)$ and $\cD^2$ only modifies $\bbP(\hat{U}_2|\hat{U}_1)$ into $\cN(2\hat{U}_1+1,1)$. Therefore, the same data would be observed if the latent variables were $\hat{U}$. Since $\hat{U}_2=U_1+U_2$, it is not possible to identify $U$ up to $\cM$-equivalence classes.
\end{example}

However, if we can still identify the DAG $\cG$ and intervention targets $I_1,...,I_K$ up to $\cM$-equivalence, then we can discover the causal structure between the interventional targets of $\cD^1,...,\cD^K$. Unfortunately, the next two examples show that this is impossible without further regularities.

\begin{wrapfigure}{r}{0.25\textwidth}
    \centering
    \vspace{-.3in}
\includegraphics[width=\linewidth]{fig/fig3.png}
\vspace{-.3in}
    \caption{An example with $p=2$ showing that there could be reversed edges between the interventional targets of $\cD^1,...,\cD^K$.} 
    \vspace{-.2in}
    \label{fig:3}
\end{wrapfigure}

\begin{example}\label{exp:3}
    Consider the data-generating process of Example \ref{exp:1}, where $I_1=\{1\}$, $I_2=\{2\}$, and $\cG=\{1\rightarrow 2\}$, illustrated in Figure \ref{fig:3} (Left). Now consider a new set of latent variables \[\hat{U}=(U_2,U_2-U_1)\] and a new function $\hat{f}(\hat{U})=(\hat{U}_1-\hat{U}_2,\hat{U}_1)$ such that $\hat{f}(\hat{U})=U=f(U)=X$. The joint distribution\footnote{The following arguments about the distribution of $\hat{U}_1$ and $\hat{U}_2$ can be derived easier if we write $U_1=\epsilon_1$ and $U_2=\epsilon_1+\epsilon_2$, where $\epsilon_1$ and $\epsilon_2$ are independent noises following $\cN(0,1)$. Then $\cD^1, \cD^2$ modify $\epsilon_1,\epsilon_2$ into $\epsilon_1'=\epsilon_1+1,\epsilon_2'=\epsilon_2+1$ respectively.} in $\cD$ has factorization $\bbP(\hat{U}_1,\hat{U}_2)=\bbP(\hat{U}_2)\bbP(\hat{U}_1|\hat{U}_2)$ by Bayes rule with $\bbP(\hat{U}_2)$ being $\cN(0,1)$ and $\bbP(\hat{U}_1|\hat{U}_2)$ being $\cN(\hat{U}_2,1)$. In addition, $\cD^1$ only modifies $\bbP(\hat{U}_1|\hat{U}_2)$ into $\cN(\hat{U}_2+1,1)$ without changing $\bbP(\hat{U}_2)$; $\cD^2$ only modifies $\bbP(\hat{U}_2)$ into $\cN(1,1)$ without changing $\bbP(\hat{U}_1|\hat{U}_2)$. Therefore, the same data would be observed if the latent variables were $\hat{U}$, the interventional targets of $\cD^1,\cD^2$ are $\hat{I}_1=\{1\},\hat{I}_2=\{2\}$ respectively, and the DAG $\hat{\cG}=\{1\leftarrow 2\}$. We thus may have reversed edges between the interventional targets, as illustrated in Figure \ref{fig:3} (Right).
\end{example}



This example shows that we may have reversed directions between the interventional targets of $\cD^1,...,\cD^K$. The next example shows that even if we have the correct partial orders between the interventional target (which implies no reversed edges), there can still be missing or excessive edges.

\begin{wrapfigure}{r}{0.3\textwidth}
    \centering
    \vspace{-.2in}
\includegraphics[width=\linewidth]{fig/fig2.png}
\vspace{-.2in}
    \caption{An example with $p=3$ showing that there could be missing or excessive edges between the interventional targets of $\cD^1,...,\cD^K$.}
    \label{fig:2}
    \vspace{-.1in}
\end{wrapfigure}


\begin{example}\label{exp:2}
    Consider a $3$-node DAG shown on the left of Figure \ref{fig:2} as $\cG$. Suppose that $f$ is the identity map and that $\cD^1,\cD^2,\cD^3$ target nodes $1,2,3$, shifting them higher by $1$, respectively. Further suppose that $\bbP(U_1)$ is $\cN(0,1)$, $\bbP(U_2|U_1)$ is $\cN(U_1,1)$, and $\bbP(U_3|U_1,U_2)$ is $\cN(U_1+U_2,1)$. Now consider the new set of variables
    \[
    \hat{U} = (U_1,U_1+U_2,U_3)
    \]
    and the function $\hat{f}(\hat{U})=(\hat{U}_1,\hat{U}_2-\hat{U}_1,\hat{U}_3)$. Then $\hat{f}(\hat{U})=U=f(U)=X$. For this, the DAG $\hat{G}$ without the edge $1\rightarrow 3$ (Figure \ref{fig:2}, Right) suffices, with $\cD^1,\cD^2,\cD^3$ shifting $\hat{U}_1,\hat{U}_2,\hat{U}_3$ by $1$ respectively. Thus, we may have missing or excessive edges between the interventional targets.
\end{example}


Note that for simplicity, we provide the above examples that can be written as linear structural equation models \cite{peters2017elements}; one can also come up with nonlinear examples. For instance, we can set the conditional distribution of $U_2$ given $U_1$ as $\cN(U_1^2,1)$ in Example \ref{exp:1} or the conditional distribution of $U_3$ given $U_1,U_2$ as $\cN((U_1+U_2)^2,1)$ in Example \ref{exp:2}. For Example \ref{exp:3}, one can use a periodic function plus constant as the structural equation and set the shift interventions to be such that they allow for an explanation with a reversed edge.

These examples show that $\langle\cG,I_1,...,I_K\rangle$ can not be identified up to $\cM$-equivalence without further regularities. To avoid these pathological cases, we propose two further assumptions. For simplicity, we defer the full discussion to Appendix~\ref{app:b} and summarize the results here. The faithfulness assumption~\ref{ass:faithfulness} rules out cases similar to Example~\ref{exp:3} and holds almost surely. In addition, Assumption~\ref{ass:3} avoids Example~\ref{exp:2}, where we can show it holds for a general class of causal DAGs, namely, directed tree graphs.
%
% We state a brief version below for simplicity, whereas a full version can be found in Appendix \ref{app:a}.
% \begin{assumption}[Informal]\label{assumption:2}
% For the observational distribution $\bbP_{U}$, we assume that  is faithful to $\cG$ and that the conditional dependency of $j$ on $i$ for $i\rightarrow j\in\cG$ can not be canceled by adding linear terms of $U_i$ to certain variables. For the interventional distributions $\bbP_{U}^{I_1},...,\bbP^{I_p}$, we assume a type of linear faithfulness, which enforces that shift on each intervention target results in a different marginal distribution of its direct children and itself, regardless of adding to itself any linear terms of variables that are not upstream of it. 
% \end{assumption}
%
Note that even under these two assumptions, $U$ still can not be identifiable up $\cM$-equivalence class. The counterexample that changes the conditional distribution of $U_2$ given $U_1$ in Example \ref{exp:1} to $\cN(U_1^2,1)$ can illustrate this. Nevertheless, we have the identifiability of $\cG,I_1,...,I_K$ up to $\cM$-equivalence classes, stated in the following theorem.

\begin{theorem}[Shift Intervention]\label{thm:1}
Suppose Assumptions \ref{assumption:1},\ref{ass:faithfulness},\ref{ass:3} hold true. If we have observational data $\cD$ and interventional data $\cD^1,...,\cD^K$ where each intervention targets
one latent node and there is at least one shift intervention on each latent node, then DAG $\cG$ and the intervention targets $I_1,...,I_K$ are identifiable up to their $\cM$-equivalence class.
\end{theorem}

The implication of this theorem is the following: given unpaired observational data $\cD$ and intervention data $\cD^1,...\cD^K$ from one shift intervention on each node, we can identify which ones of $\cD^1,...\cD^K$ correspond to intervening the same latent node as well as the causal structure between them. For example, given high-dimensional single-cell transcriptomic readout from knocking down genes $g_1,...,g_n$, we are able to figure out which genes belong to the same group (which can be interpreted as programs) and the causal structure (which can be interpreted as regulatory relationships) between them. We will further illustrate this example in Section~\ref{sec:experiments}.

==> content/old/introduction-old.tex <==
\section{Introduction}
%{\color{red} sprinkle in some citations}
\todo{we can motivate the unpaired setting here if needed}
\todo{update the discussion to include faithfulness}

The problem of discovering causal structures from observational and interventional data is important in many fields including statistics, biology, sociology, and economics (\tbd{cite}). 
%
Directed acyclic graph (DAG) models allow one to reason about causal questions such as predicting the effect of interventions as well as the estimation of counterfactuals \cite{pearl2009causality}. 
%Causal models have seen wide application to problems in statistics, biology, social science, machine learning, and many others.
%
Traditional causal structure learning is limited to the setting where the causal variables are observed \cite{heinze2018causal}. 
%
While sufficient in many applications, this restriction is limiting in most regimes where the available datasets are either perceptual (e.g., images) or very-high dimensional (e.g., the expression of $>20k$ human genes).
%higher dimensional regimes which are common in machine learning and genetics. 
%
In an imaging dataset, learning a causal graph on the pixels themselves would not only be difficult since there is no common coordinate system across images (pixel $i$ in one image may have no relationship with pixel $i$ in another image) but of questionable utility due to the relative meaninglessness of interventions on individual pixels. 
%
Similar problems are also present when working with very high-dimensional data.
%
For example, in a gene-expression dataset, subsets of genes (e.g. belonging to the same pathway) may function together to induce other variables and should therefore be aggregated into one causal variable.

% For example, in an image dataset, the only observed variables are the pixel values. Learning a causal graph on the pixels themselves would not only be difficult, but of questionable utility due to the lack of interpretability and relative meaninglessness of the associated interventions. 

This means that the causal variables need to be learned.
%
The recent field of latent causal representation learning \cite{cai2019triad,xie2022identification,kivva2022identifiability} seeks to remedy this issue by recovering a causal representation in \emph{latent} space, i.e. a small number of variables $U$ that are then mapped to the observed samples in the ambient space via some mixing map $f$. 
%
When successful, this framework could allow for much more semantically meaningful latent factors, in particular those that correspond to interventions of interest to the modeler.
%
Returning to the image and the genomic examples, latent factors could for example be abstract functions of pixels (corresponding to objects) or groups of genes (corresponding to pathways).


Despite a recent flurry of interest, latent causal representation learning remains challenging. 
%
First, it inherits the difficulties of causal structure learning where the possible number of causal DAGs grows super exponentially in the latent dimension.
%
Moreover, since we only observed the variables after the unknown mixing function but never the latent variables, it is generally impossible to recover the latent causal representations with only observational data.
%
For example, assuming the causal DAG is the empty graph, such unidentifiability has been discussed in previous disentanglement works (\tbd{cite}).
%
However, recent advances in many applications enable the possibility to generate interventional data.
%
As an example, in genomics, we can genetically perturb single or several genes through pooled CRISPR experiments (\tbd{cite}).
%
Such interventional data can be used to identify the causal variables and learn the underlying rules.

% In particular, it is generally nontrivial to demonstrate that recovered latent causal representations correspond to the ground truth. \cite{ahuja2022interventional} proved identifiability in the setting of hard interventions, when the embedding is a polynomial and data from all single-node interventions are provided. 
%prior work
%For causal representation learning, \cite{cohen2022towards} argues that rather than focusing on \emph{identifiability} of the latent variables, the focus should be instead on \emph{admissibility}, in other words the ability to predict the outcome of (unseen) interventions and (unseen) compositions of interventions.
%setting: unpaired data, as motivated by e.g. single-cell applications
%somewhere - approach: generate intervention samples from observational samples 

In this work, we establish identifiability results for \emph{soft shift} interventions, an intervention type of significant interest to biological applications.
%
We also extend the identifiability for \emph{deterministic hard} interventions in previous work \cite{ahuja2022interventional} to the identifiability of the causal DAG.
%
The identifiability is up to an equivalence class, which describes the indeterminacy that can not be resolved.
%
It then remains to design an algorithmic approach to estimate the latent causal representation from data. 
%
We propose an autoencoding variational Bayes framework that directly encodes the graph structure in the latent space, allowing for in-architecture simulation of counterfactual copies of observational samples. 
%This yields an architecture where observational samples are encoded into the independent latent exogenous factors of the latent structural causal model, propagated through the intervention-modified graphical model to recover the latent variables, and finally decoded into the ambient space to form interventional samples. 
This explicit approach 
%in contrast to VAE approaches such as in \cite{ahuja2022interventional} that do not encode the graph)
crucially allows for generalization from training on single-node interventions to multiple-node interventions. 
%
The primary challenge in designing the autoencoding variational Bayes framework is that the observational and interventional data are not \emph{paired}, i.e., we do not know what an interventional sample would look like if it had not been intervened upon.
%
This precludes computing the counterfactual likelihood;
%comparing the generated counterfactual interventional samples to the dataset of interventional samples. 
%
instead, we use a \emph{discrepancy measure} to directly compare the distributions of the simulated and ground truth interventional data. 
%In our experiments, we focused on the maximum mean discrepancy (MMD), showing that this choice in certain instances yields a loss that lower bounds the model loglikelihood.
%
We show theoretically that this leads to a valid lower bound of the counterfactual likelihood and the framework is consistent under certain conditions.
%
Finally, we apply our approach to both synthetic and
real-world genomics datasets.
%why VAE - better for fitting distributions (?) and easier to disentangle latent exogenous variables

%This paper is organized as follows: We introduce our model for causal representation learning in Section \ref{sec:setup}, and prove identifiability results for shift interventions in Section \ref{sec:identifiability}. In Section \ref{sec:VAE} we introduce our discrepancy-based VAE for learning the causal representation, and in Section \ref{sec:experiments} we present experimental results on synthetic and biological data.

\subsection{Related Work}

\textbf{Identifiable Representation Learning.}
%
The identifiability of latent representations from observed data has been a subject of ongoing study \cite{comon1994independent,hyvarinen2019nonlinear,khemakhem2020variational}.
%
A common assumption is that the latent variables are either independent, conditionally independent given some observed variable, or follow a known distribution \cite{zimmermann2021contrastive}.
%
In contrast, we do not make any independence assumptions on the latent variables or assume that we know their distribution a priori.
%
Instead, we assume that the variables are related via a causal DAG model, and use data from interventions on the latent variables in order to identify the representation.

\textbf{Causal Structure Learning.}
%
The recovery of a causal DAG from data is well-studied for the setting where the causal representation is directly observed \cite{heinze2018causal}.
%
Methods for this task take a variety of approaches, including exact search \cite{cussens2020gobnilp} and greedy search \cite{chickering2002optimal} to maximize a score such as the posterior likelihood of the DAG, or an approximation thereof.
%
These scores can be generalized to incorporate interventional data \cite{kuipers2022interventional}, and methods can often be naturally extended by considering an augmented search space \cite{mooij2020joint}.
%
Indeed, interventional data is generally necessary for identifiability without further assumptions on the functions relating variables \cite{squires2022causal}.

The task of identifying a causal DAG over a latent causal representation is less well-studied, but has become the focus of a flurry of recent work \cite{cai2019triad,xie2022identification,kivva2022identifiability}.
%
These works largely do not consider interventions, and thus require restrictions on functional forms as well as sparsity assumptions on the map $f$ from the latent variables to the observed variables.
%
Among works that do not restrict the map $f$, \cite{ahuja2022weakly} and \cite{brehmer2022weakly} assume access to \textit{paired} counterfactual data.
%
In contrast, we consider only \textit{unpaired} data, which is more common in applications such as biology \cite{stark2020scim}.
%
Unpaired interventional data is considered by \cite{ahuja2022interventional}, \cite{seigal2022linear}, and as a special case of \cite{liu2022weight}.
%
Our work builds on and complements these results by extending their identifiability to \textit{shift} interventions, which are commonly used to model genetic perturbations in biology \cite{zhang2021matching}, and by offering a score-based learning algorithm based on variational Bayes.

\textbf{Autoencoding Variational Bayes.} Autoencoding variational Bayes (AVB) \cite{kingma2013auto}, while originally proposed to learning and inference in deep Gaussian latent variable model, has since been adapted for other probabilistic graphical models \cite{johnson2016structured, srivastava2017autoencoding, dieng2016topicrnn, xu2019variational}. In order to apply AVB to an arbitrary graphical model, it needs to be converted into a variational autoencoder \cite{kingma2013auto, rezende2014stochastic} first. This involves introducing a deep neural network (encoder) that parameterizes the variational posterior distribution over the latent variables of the graphical model and a decoder network, that parameterizes the actual graphical model. This step reduces the tasks of learning and inference in the original graphical model to that of learning the parameters of the encoder and decoder model. However, deep neural network based parameterization from this step often leads to intractability of the evidence under the model. Therefore, AVB prescribes a scheme to derive a tractable lower-bound to the evidence (ELBO) using a number of model-specific reparameterization tricks \cite{williams1992simple} to ensure differentiability of the ELBO. With a tractable learning objective, gradient-based training methods, such as stochastic gradient descent, can be deployed to learn model parameters and carry out amortized variational inference on the latent variables.
